Consistent Multiclass Algorithms for Complex Metrics and Constraints

We present consistent algorithms for multiclass learning with complex performance metrics and constraints, where the objective and constraints are defined by arbitrary functions of the confusion matrix. This setting includes many common performance metrics such as the multiclass G-mean and micro F1-measure, and constraints such as those on the classifier's precision and recall and more recent measures of fairness discrepancy. We give a general framework for designing consistent algorithms for such complex design goals by viewing the learning problem as an optimization problem over the set of feasible confusion matrices. We provide multiple instantiations of our framework under different assumptions on the performance metrics and constraints, and in each case show rates of convergence to the optimal (feasible) classifier (and thus asymptotic consistency). Experiments on a variety of multiclass classification tasks and fairness-constrained problems show that our algorithms compare favorably to the state-of-the-art baselines.

==> con-ellipsoid-proof_old.tex <==
\begin{thm*}[(Restated) Convergence of Conellipsoid]
Fix $\epsilon \in (0,1)$. 
Let $\psi, \phi_1,\ldots,\phi_K: [0,1]^d\>[0,1]$ be convex and $L$-Lipschitz w.r.t. the $\ell_2$ norm. Let $\Omega$ in Algorithm \ref{alg:GDA-con} be a $(\rho , \rho', \delta)$-approximate LMO for sample size $N$. Suppose the strict feasibility condition in Assumption \ref{assp:strict-feasibility} holds for radius $r>0$. Let the initial classifier $h^0$ satisfy this condition, i.e. $\bphi(\C[h^0]) \leq -r$ and $\C[h^0]=\C^0$. Let $\bar{d}=d+K$. Let $\bar{h}$ be the classifier returned by Algorithm \ref{alg:ellipsoid-con} when run for $T$ iterations with  initial radius $a>2(L+\frac{L+1}{r})$ and approximation factor $\tau> a(\rho+2\sqrt{d}\rho')$.
 Then with probability $\geq 1 - \delta$ over draw of $S \sim D^N$, after $T = \cO\left(\bar{d}^2 \log\left(\bar{d}/{\epsilon}\right)\right)$ iterations:
\begin{align*}
\textbf{Optimality:}~~\psi(\C[\bar{h}]) \,&\leq\, \min_{\C\in\cC:\, \phi_k(\C) \leq 0,\forall k}\,\psi(\C) + \cO\left(\epsilon + \bar{d} \sqrt{\tau} \right);   \\
\textbf{Feasibility:}~~\phi_k(\C[\bar{h}]) \,&\leq\, \tau ,~\forall k \in [K].
\end{align*}
 
\end{thm*}


The core ellipsoid algorithm theorem we will use is stated below. The proof is a simple extension of the standard ellipsoid algorithm argument to work with shallow cuts \citep{Bubeck15}.
\begin{thm}
\label{thm:ellipsoid-volumes}
Let $H_0 \in \R^{d\times d}$ be a positive definite matrix. Let $\c_0, \w\in \R^d$ and $\gamma \in \R_+$. Let $A$ be an ellipsoid, and $B$ be a half space containing the centre of $A$ given as follows
\begin{align*}
A &= \{ \x \in \R^d : (\x- \c_0)^\top H_0^{-1} (\x-\c_0) \leq 1\} \\
B &= \{ \x \in \R^d : \w^\top (\x- \c_0) \leq \gamma \sqrt{\w^\top H_0 \w } \}.
\end{align*}
Let $\c_1\in\R^d, H_1\in \R^{d \times d}$ be given as follows:
\begin{align*}
    \c_1 &= \c_0 - \frac{1-d\gamma}{(d+1)\sqrt{\w^\top H_0 \w }} H_0 \w  \\
    H_1^{-1} &= H_0^{-1/2} \left(H \right)^{-1} H_0^{-1/2},
 \end{align*}
where $H^{-1} = a \widetilde \w \widetilde \w^\top + b(I - \widetilde \w \widetilde \w^\top)$, with $\widetilde \w = \frac{1}{\sqrt{\w^\top H_0 \w }} H_0^{1/2}\w$. The scalars $a$ and $b$ are given as $a=\frac{1}{(1-t)^2}$ and $b=\frac{(1-t)-(\gamma+t)^2}{(1-t)^2-\gamma^2(1-t)^2}$ with $t=\frac{1-d\gamma}{d+1}$.
 
Then the ellipsoid given by
\[
C = \{ \x \in \R^d : (\x- \c_1)^\top H_1^{-1} (\x-\c_1) \leq 1\}
\]
is a superset of $A \cap B$, and the ratio of volumes of $C$ and $A$ is upper bounded by $\exp\left( \frac{-1}{2d}+\gamma \right)$.
\end{thm}




We will define some functions and variables below that will be useful in our proofs:
\begin{align*}
\cL^\con (\C, \bxi , \blambda, \bmu) &= \psi(\bxi) + \blambda^\top (\C - \bxi) + \bmu ^\top \bphi(\bxi) \\
f^\con (\blambda, \bmu) &= \min_{\C \in \cC, \bxi \in \Delta_d} \cL^\con (\C, \bxi , \blambda, \bmu) \\
\widehat f^\con (\blambda, \bmu)& = f^\con (\blambda, \bmu) - \infty \1( \|[\blambda,\bmu]\|_2 > a) -\infty \1( \bmu < 0 ) \\
\bxi(\blambda, \bmu) &\in \argmin_{\bxi \in \Delta_d} \psi(\bxi) - \blambda^\top \bxi + \bmu ^\top \bphi(\bxi) 
\end{align*}
The helper function $\widehat f^\con (\blambda, \bmu)$ is simply equal to $ f^\con (\blambda, \bmu)$ when its arguments $(\blambda,  \bmu)$ are within the ball of radius $a$ and $\bmu$ is non-negative. Otherwise it is equal to negative infinity. The algorithm ensures that $\blambda^t, \bmu^t$ lies within this region, whenever the LMO $\Omega$ is called (reaches the else condition on line 9). And for all such $t$, we have $\widehat f^\con (\blambda^t, \bmu^t) =  f^\con (\blambda^t, \bmu^t)$.

Consider an iteration $t$ such that $\widehat f^\con (\blambda^t, \bmu^t) =  f^\con (\blambda^t, \bmu^t)$. Let  $\bxi(\blambda^t, \bmu^t)=\bxi^t$, where $\blambda^t, \bmu^t$ are the iterates in Algorithm \ref{alg:ellipsoid-con}. We have that
\begin{align}
    {\blambda^t}^\top \C[h^t] &\leq \min_{\C \in \cC} {\blambda^t}^\top \C + \|\blambda^t\|_\infty  \rho  \leq \min_{\C \in \cC} {\blambda^t}^\top \C + a  \rho \\
    \|\C[h^t] - \C^t \|_2 &\leq \sqrt{d} \rho' \\
    {\blambda^t}^\top \C^t &= {\blambda^t}^\top (\C^t-\C[h^t]) + {\blambda^t}^\top \C[h^t] \nonumber \\
    &\leq \|\blambda^t\|_2 \|\C^t - \C[h^t]\|_2 +  \min_{\C \in \cC} {\blambda^t}^\top \C + a\rho \nonumber \\
    &\leq \min_{\C \in \cC} {\blambda^t}^\top \C + a(\rho+\sqrt{d}\rho'),
\end{align}
where $h^t$ and $\C^t$ are the iterates in Algorithm \ref{alg:ellipsoid}.  The first two inequalities above are simply a restatement of the $(\rho,\rho',\delta)$-approximate property of the LMO. Note that the above inequalities hold only with probability $1-\delta$ (over draw of $S \sim D^N$) uniformly for all $t$. The rest of the analysis will only apply for this high probability event.


Let $(\blambda^*, \bmu^*)$ be a maximizer of $f^\con$ over $\R^d \times \R_+^K$. From Lemma \ref{lem:gda-con-helper} we have that $ \|[\blambda^*,\bmu^*]\|_2 \leq L + \frac{L+1}{r} \leq a/2$. Thus:
\begin{equation}
\max_{\blambda \in \R^d, \bmu \in \R^K_+} f^\con(\blambda, \bmu) = \max_{\blambda \in \R^d, \bmu \in \R^K_+} \widehat f^\con(\blambda, \bmu) = 
\psi(\C^*) = \min_{\C \in \cC, \bphi(\C) \leq 0} \psi(\C).
\label{eqn:dual-optimizer-bounded}
\end{equation}
This ensure that the initial ellipsoid (ball of radius $a$) contains $(\blambda^*, \bmu^*)$.

We break the proof of the theorem into multiple lemmas below. The proof has two main parts. 
\begin{itemize}
    \item  In the first part (Lemmas \ref{lem:con-ellipsoid-f-supergradient}, \ref{lem:con-ellipsoid-separating-hyperplane}, \ref{lem:con-ellipsoid-f-lipschitz} and Theorem \ref{thm:ellipsoid-dual-con}), we show that even with an approximate LMO, the iterates $\blambda^t$ approximately maximize $\widehat f^\con$.  
    \item In the second part (Lemmas \ref{lem:dual-to-primal-1} and \ref{lem:dual-to-primal-2}), we show how the post-processing step in line 14 of the algorithm converts the approximate maximization guarantee on $\widehat f^\con$ into a minimization guarantee for the original constrained primal problem.
\end{itemize}

\subsubsection{Approximate maximization of $\widehat f^\con$}
We begin by showing that $\q_t = [\C^t - \bxi^t, \bphi(\bxi^t)] \in \R^{d+K}$ is an approximate super-gradient of the function $\widehat f^\con$.
% \todoharish{Subscript all norms}

\begin{lem}
\label{lem:con-ellipsoid-f-supergradient}
Let $t$ be such that $\|[\blambda^t,\bmu^t]\|_2\leq a$ and $\bmu^t \geq 0$. Then, $[\C^t - \bxi^t, \bphi(\bxi^t)]$ is an $\epsilon$-supergradient to $\widehat f^\con$ at $\blambda^t$, with $\epsilon=a(\rho+2\sqrt{d}\rho') $, i.e. for  all $\blambda \in \R^d, \bmu \in \R^K$, 
\[
\widehat f^\con(\blambda, \bmu) 
\leq 
\widehat f^\con(\blambda^t, \bmu^t) + (\blambda - \blambda^t)^\top (\C^t -\bxi^t) +
(\bmu - \bmu^t)^\top (\bphi(\bxi^t)) + \epsilon
\]
\end{lem}
\begin{proof}
Fix $\blambda, \bmu$ such that $\| \blambda, \bmu \|_2 \leq a $ and $\bmu\geq 0$. 
\begin{align*}
\widehat f^\con(\blambda, \bmu)  
&= \min_{\C \in \cC, \bxi \in \Delta_d} \cL(\C,\bxi, \blambda, \bmu) \\
&\leq  \cL(\C[h^t],\bxi^t, \blambda, \bmu) \\
&= \cL(\C^t,\bxi^t, \blambda, \bmu) + (\C[h^t] - \C^t)^\top \blambda \\
&\leq \cL(\C^t,\bxi^t, \blambda, \bmu) + \|\C[h^t] - \C^t\|_2 \|\blambda\|_2 \\
& \leq \cL(\C^t,\bxi^t, \blambda, \bmu) + a\sqrt{d}\rho'.
\end{align*}
We further have:
\begin{align*}
\widehat f^\con(\blambda^t, \bmu^t)  
&= \min_{\C \in \cC} {\blambda^t}^\top \C + \min_{\bxi \in \Delta_d} \psi(\bxi) -  {\blambda^t}^\top \bxi + {\bmu^t}^\top \bphi(\bxi) \\
&\geq {\blambda^t}^\top \C^t - a (\rho+\sqrt{d}\rho') + \psi(\bxi^t) -  {\blambda^t}^\top \bxi^t + {\bmu^t}^\top \bphi(\bxi^t) \\
&= \cL(\C^t, \bxi^t, \blambda^t, \bmu^t) - a(\rho+\sqrt{d}\rho') \\
&= \cL(\C^t, \bxi^t, \blambda, \bmu) + (\blambda^t - \blambda)^\top (\C^t - \bxi^t) + (\bmu^t - \bmu)^\top \bphi(\bxi^t) - a(\rho+\sqrt{d}\rho')  \\
&\geq \widehat f^\con(\blambda, \bmu)  - a\sqrt{d} \rho' + (\blambda^t - \blambda)^\top (\C^t - \bxi^t) + (\bmu^t - \bmu)^\top \bphi(\bxi^t) - a(\rho+\sqrt{d}\rho'),
\end{align*}
as desired.
\end{proof}

Now we can show that the JLE subroutine (Algorithm \ref{alg:jle}), when called by Algorithm \ref{alg:ellipsoid-con} at iteration $t$, only excludes $\blambda, \bmu$ which are ``worse'' than the current iterate $\blambda^t, \bmu^t$. 
%
\begin{lem}
 \label{lem:con-ellipsoid-separating-hyperplane}
 Let $t$ be such that $\|[\blambda^t,\bmu^t]\|_2 \leq a$ and $\bmu^t \geq 0$. Let 
 \begin{align*}
    A_t &= \{\bu, \bv \in \R^d \times \R^k : \widehat f^\con(\bu,\bv) \geq \widehat f^\con(\blambda^t, \bmu^t) \} \\
    B_t &= \{ \bu, \bv \in \R^d\times \R^k: \bu^\top (\C^t - \bxi^t) + \bv^\top\bphi(\bxi^t) \geq {\blambda^t}^\top (\C^t - \bxi^t) + {\bmu^t}^\top \bphi(\bxi^t) - a(\rho+2\sqrt{d}\rho') \}.
 \end{align*}
 Then $A_t \subseteq B_t$.
\end{lem}
\begin{proof}
Let $\bu, \bv \in \R^d \times \R^k$. Then by Lemma \ref{lem:con-ellipsoid-f-supergradient}, we have
\begin{align*}
\widehat f^\con(\bu, \bv) 
&\leq 
\widehat f^\con(\blambda^t, \bmu^t) + (\bu - \blambda^t)^\top (\C^t -\bxi^t) +
(\bv - \bmu^t)^\top (\bphi(\bxi^t)) + a(\rho+2\sqrt{d}\rho').
\end{align*}
%
Let $(\bu,\bv) \in A_t$, then we have
\[
 (\bu - \blambda^t)^\top (\C^t -\bxi^t) +
(\bv - \bmu^t)^\top (\bphi(\bxi^t)) + a(\rho+2\sqrt{d}\rho')  \geq 0.
\]
Thus we have that $(\bu,\bv) \in B_t$.
\end{proof}

We will also need the Lipschitzness of $f^\con$ to prove the convergence of the ellipsoid algorithm. 
\begin{lem}
\label{lem:con-ellipsoid-f-lipschitz}
$f^\con$ is a $1$-Lipschitz function w.r.t. $\ell_1$ norm. 
\end{lem}
\begin{proof}
The difference $f^\con$ at 
$\blambda, \bmu$ and $\blambda',\bmu'$ can be bounded by:
\begin{align*}
f^\con(\blambda, \bmu) - f^\con(\blambda',\bmu') 
&= \min_{\C\in\cC, \bxi \in \Delta_d} \cL^\con(\C, \bxi, \blambda, \bmu) - \min_{\C\in\cC, \bxi \in \Delta_d} \cL^\con(\C, \bxi, \blambda', \bmu') \\
&\leq \max_{\C\in\cC, \bxi \in \Delta_d} \left(
\cL^\con(\C, \bxi, \blambda, \bmu)  -   \cL^\con(\C, \bxi, \blambda', \bmu') \right) \\
&\leq  \max_{\C\in\cC, \bxi \in \Delta_d}  
\left(   (\blambda - \blambda')^\top (\C - \bxi) + (\bmu - \bmu')^\top \bphi(\bxi) \right) \\
&\leq  \max_{\C\in\cC, \bxi \in \Delta_d} \left( \|\blambda - \blambda'\|_1 \|\C - \bxi\|_\infty + \|\bmu - \bmu'\|_1 \|\bphi(\bxi)\|_\infty \right) \\
&\leq \|\blambda - \blambda'\|_1 +  \|\bmu - \bmu'\|_1,
\end{align*}
which proves the $1$-Lipschitz property of $f^\con$.
\end{proof}



When the norm of the approximate supergradient $\q_t=[ \C^t - \bxi^t, \bphi(\bxi^t)]$ is small, we can bound the suboptimality of the iterate $\blambda^t, \bmu^t$ as follows.

\begin{lem}
\label{lem:con-ellpsoid-small-grad-implies-close-to-optim}
Let $t$ be such that $\|[\blambda^t,\bmu^t]\|\leq a$ and $\bmu^t \geq 0$. For any $\alpha>0$, 
\[
\|[ \C^t - \bxi^t, \bphi(\bxi^t)] \|_2  \leq \alpha \Rightarrow \widehat f^\con(\blambda^t, \bmu^t) \geq \max_{\blambda\in \R^d, \bmu \in \R_+^K} f(\blambda, \bmu)  - a(\rho+2\sqrt{d}\rho'+2\alpha).
\]
\end{lem}
\begin{proof}
Let $\blambda^*, \bmu^* \in \argmax_{\blambda, \bmu \in \R^d \times \R_+^K} \widehat f^\con(\blambda, \bmu)$. From Lemma \ref{lem:con-ellipsoid-f-supergradient}, we have
\begin{align*}
\widehat  f^\con(\blambda^*, \bmu^*) 
&\leq \widehat f^\con(\blambda^t, \bmu^t) + (\blambda^* - \blambda^t)(\C^t - \bxi^t) + (\bmu^* - \bmu^t) (\bphi(\bxi^t)) + a(\rho+2\sqrt{d}\rho') \\
&\leq  \widehat f^\con(\blambda^t, \bmu^t) + \|[\blambda^* - \blambda^t, \bmu^* - \bmu^t\|_2 \|[ \C^t - \bxi^t, \bphi(\bxi^t)] \|_2 + a(\rho+2\sqrt{d}\rho') \\
&\leq  \widehat f^\con(\blambda^t, \bmu^t) + 2a\alpha + a(\rho+2\sqrt{d}\rho'),
\end{align*}
as desired.
\end{proof}


We can now show that the iterates $\blambda^t, \bmu^t$ effectively approach a maximizer of $\widehat f^\con$ .
\begin{thm}
\label{thm:ellipsoid-dual-con}
Let the assumptions stated in Theorem \ref{thm:ellipsoid-con} hold. Let $T>12(\bar{d})^2$. Then,
\[
\max_{0 \leq t\leq T} \widehat f^\con({\blambda^t, \bmu^t}) \geq \max_{\blambda, \bmu} \widehat f^\con(\blambda, \bmu) - \nu
\]
where $\bar{d}=d+K$, and $\nu =  4a \sqrt{d+K} \exp\left(-\frac{T}{4(d+K)^2}\right) + 4a\sqrt{(d+K)\tau} +  \tau + 8(d+K) \sqrt{\tau}$.
\end{thm}
\begin{proof}

Consider some iteration $t$ of Algorithm \ref{alg:ellipsoid-con}. Let the operating ellipsoid at iteration $t$ be denoted by $E_t$, i.e.,
\[
E([\blambda^t, \bmu^t], \A^t) = E_t = \{\bu, \bv \in \R^d \times \R^k: ([\bu, \bv] - [\blambda^t, \bmu^t])^\top [\A^t]^{-1} ([\bu, \bv] - [\blambda^t, \bmu^t]) \leq 1 \} 
\]

At initialization, $E_0$ is equal to the $\ell_2$-norm ball of radius $a$, which is large enough to contain a maximiser $\blambda^*, \bmu^*$ of $\widehat f^\con$. 
If the iterate $\blambda^t, \bmu^t$ falls in the region where $\widehat f$ is negative infinity, an appropriate hyperplane separating $\blambda^t, \bmu^t$ from the finite region of $\widehat f^\con$ is given to the John-Lowner ellipsoid construction sub-routine. (Lines 5 to 8 of the  algorithm). Thus $E_{t+1}$ is clearly a superset of $E_t \cap \{[\bu,\bv]: \widehat f^\con(\bu,\bv) \geq \widehat f^\con (\blambda^t, \bmu^t) \}$.

On the other hand, if $\blambda^t, \bmu^t$ falls in the finite region of $\widehat f^\con$, by virtue of the approximation factor $\tau > a(\rho+2\sqrt{d}\rho')$, the property of the John-Lowner ellipsoid  and from Lemma \ref{lem:con-ellipsoid-separating-hyperplane}, we have
\[
E_{t+1} \supseteq E_{t} \cap B_t \supseteq E_t \cap A_t = E_t \cap \{[\bu,\bv]: \widehat f^\con(\bu,\bv) \geq \widehat f^\con (\blambda^t, \bmu^t) \},
\]
where $A_t, B_t$ are as defined in Lemma \ref{lem:con-ellipsoid-separating-hyperplane}.

Thus, in all three cases, 
\[
E_{t+1}
\supseteq
E_t \cap \{[\bu,\bv]: \widehat f^\con(\bu,\bv) \geq \widehat f^\con (\blambda^t, \bmu^t) \}.
\]
Furthermore, $E_t$ contains the maximizers of $\widehat f^\con$ for all $t$.

The key tool for arguing the convergence of the ellipsoid algorithm is the shrinking volume of the ellipsoids.  In Algorithm \ref{alg:ellipsoid-con}, when the iterate $\blambda^t, \bmu^t$ falls outside the region where $\widehat f^\con$ is finite, the shrinking of volume of the ellipsoid simply follows from Theorem \ref{thm:ellipsoid-volumes} as the tolerance $\gamma$ is equal to $0$. We will now argue that the volume of $E_{t+1}$ shrinks even otherwise, unless the iterate $\blambda^t, \bmu^t$ is already close to a maximizer $\blambda^*, \bmu^*$ of $\widehat f^\con$.

To this end, let $\q_t = [(\C^t - \bxi^t), \bphi(\bxi^t)] \in \R^{d+K}$.  Let $\gamma_t = \frac{\tau}{\sqrt{\q_t^\top  [\A^t] \q_t}}$.  If the iterates $\blambda^t,\bmu^t$ falls outside the region where $\widehat f^\con$ is finite, then $\C^t,  \bxi^t$ are undefined, but $\gamma_t$ can be taken to be $0$. We will consider two cases.
~\\[-5pt]

\noindent \textbf{Case 1}: $\gamma_t \leq \frac{1}{4(d+K)}$ for all $t \in [T]$. 

Denote by $\|\x\|_\A $ as the norm of $\x$ in the inner product given by $\A^{-1}$, i.e. $\|\x\|_\A = \sqrt{\x^\top \A^{-1} \x}$. Let $\A=\A^{T+1}$ for the analysis of this case. 
From Theorem \ref{thm:ellipsoid-volumes}, we have that the volume of $E_{T+1}$ is at most $\exp\left(-\frac{T}{4(d+K)}\right)$ times the volume of $E_0$. Hence, at least one of the principal axes of $E_{T+1}$ must have a length of less than $a \cdot \exp(-\frac{T}{4(d+K)^2})$. Let this axis be $[\bu,\bv]$, i.e. $\|[\bu,\bv]\|_\A^2 = [\bu,\bv]^\top [\A^{T+1}]^{-1} [\bu, \bv]=1$ and $\|[\bu, \bv]\| \leq a \cdot \exp(-\frac{T}{4(d+K)^2})$. 


We will assume without loss of generality that $\bv^\top \bv_+ \geq \|\bv\|^2/2$, where $\bv_+$ is the positive part of the vector $\bv$. This is valid because $\bv \top \bv_+ + (-\bv)^\top (-\bv)_+ = \|\bv\|^2$ and if $[\bu, \bv]$ is  an axis direction of the ellipsoid $E_{T+1}$ (or eigen vector of $\A^{T+1}$), then so is $[-\bu,-\bv]$. Let $[\bu, \bv_+]$ be decomposed  as $\alpha [\bu, \bv] + \beta \w$, where $\w\in \R^{d+K}$ is orthogonal to $[\bu,\bv]$. We would then have that $\alpha=\frac{[\bu,\bv_+]^\top[\bu,\bv]}{\|[\bu,\bv]\|^2} \geq \frac{\|\bu\|^2+\|\bv\|^2/2}{\|\bu\|^2+\|\bv\|^2}\geq \frac{1}{2}$. As $[\bu,\bv]$ is an eigenvector of $\A$, we have that  $\w$ is also $\A^{-1}$ orthogonal to $[\bu,\bv]$, i.e. $\w^\top \A^{-1}[\bu,\bv]=0$.

Let $\blambda'=\blambda^* + 4\bu$, and $\bmu' = \bmu^* + 4\bv_+$.  We now argue that $[\blambda', \bmu']\in E_0 \setminus E_{T+1}$ and $\bmu' \geq \0$.  Clearly, $\bmu' \geq \0$ as $\bmu^*$ and $\bv_+$ are greater than $\0$.  We also have that
$\|[\blambda', \bmu']\| \leq \|[\blambda^*, \bmu^*]\|+4\|[\bu,\bv_+]\| \leq \frac{a}{2} + 4 \|[\bu, \bv]\| \leq a\left( \frac{1}{2} + 4 \exp(-\frac{T}{4(d+K)^2}) \right) \leq a(0.5+4e^{-3}) \leq a$. Thus $(\blambda',\bmu') \in E_0$. 

Further,
\begin{align*}
\|[\blambda',\bmu']- [\blambda^{T+1},\bmu^{T+1}\|_\A
&\geq 
\|[\blambda', \bmu']- [\blambda^*, \bmu^*]\|_\A - \|[\blambda^*, \bmu^*]- [\blambda^{T+1}, \bmu^{T+1}] \|_\A \\
&\geq 
\|[\blambda', \bmu']- [\blambda^*, \bmu^*] \|_\A - 1 =4\|[\bu,\bv_+]\|_\A - 1 \\
&= 4\|\alpha [\bu,\bv]+\beta \w \|_\A - 1 \\
&= 4\alpha\| [\bu,\bv] \|_\A + 4\beta \|\w\|_\A - 1 \\
&\geq 4\alpha\| [\bu,\bv] \|_\A - 1 
% \\
% &=
~=
4\alpha - 1 
% \\
% &
~\geq 1.
\end{align*}
Thus $[\blambda',\bmu']\notin E_{T+1}$.

All points in $E_0 \setminus E_{T+1}$ are worse (i.e. have a smaller $\widehat f^\con$ value) than $[\blambda^{t}, \bmu^t]$ for some $t$ as it was discarded by the JLE procedure at step $t$. We thus have:
% $[\blambda', \bmu'] \notin E_{T+1}$ that is such that $\|[\blambda',\bmu'] - [\blambda^*, \bmu^*]\|_2$ is less than $a \cdot \exp(-\frac{T}{4(d+K)^2})$,  but is such that $f^\con(\blambda', \bmu')<f^\con(\blambda^T, \bmu^T)$.  Thus, we have
\begin{align}
    \max_{0\leq t \leq T} \widehat f^\con(\blambda^t, \bmu^t) &\geq \widehat f^\con(\blambda', \bmu') = f^\con(\blambda',\bmu') \nonumber \\
    f^\con(\blambda', \bmu') &\geq f^\con(\blambda^*,\bmu^*) -  \|[\blambda', \bmu'] - [\blambda^*, \bmu^*]\|_1 \nonumber \\
     & \geq f^\con(\blambda^*, \bmu^*) - \sqrt{d+K} \|[\blambda', \bmu'] - [\blambda^*, \bmu^*]\|_2 \nonumber \\
    &\geq  f^\con(\blambda^*,\bmu^*) - 4a \sqrt{d+K}  \| [\bu, \bv]\|   \nonumber \\
     &\geq  f^\con(\blambda^*,\bmu^*) - 4a \sqrt{d+K} \exp\left(-\frac{T}{4(d+K)^2}\right)   \nonumber \\
    \max_{0\leq t \leq T} \widehat f^\con(\blambda^t, \bmu^t) &\geq \widehat f^\con(\blambda^*, \bmu^*) - 4a \sqrt{d+K} \exp\left(-\frac{T}{4(d+K)^2}\right),
    \label{eqn:dual-subop-case1}
\end{align}
where the second inequality is due to the Lipschitzness of $f^\con$ w.r.t.\  the $\ell_\1$ norm (Lemma \ref{lem:con-ellipsoid-f-lipschitz}).
~\\[-5pt]

\noindent\textbf{Case 2}:  $\gamma_t > \frac{1}{4(d+K)}$ for some $t\in{0,1,\ldots,T}$.

In this case,
\begin{align*}
   \q_t^\top \A^t \q_t \leq 16(d+K)^2 \tau^2.
\end{align*}
We thus have that $\|\q_t\|^2 \leq 4(d+K)\tau$ or the smallest eigen value of $\A^t$ is less than $4(d+K)\tau$. 

If $\|\q_t\| \leq 2\sqrt{(d+K)\tau}$ then by Lemma \ref{lem:con-ellpsoid-small-grad-implies-close-to-optim} we have that
\begin{align}
    \widehat f^\con(\blambda^t, \bmu^t) 
    &\geq  \widehat f^\con(\blambda^*, \bmu^*) - a(\rho+2d\rho'+4\sqrt{(d+K)\tau}) \nonumber\\
    &\geq  \widehat f^\con(\blambda^*, \bmu^*) - 4a\sqrt{(d+K)\tau} -  \tau. \label{eqn:dual-subop-case2a}
\end{align}

If the smallest eigen value of $\A^t$ is less than $4(d+K)\tau$, then one of the principal axes of the ellipsoid $E_t$ has length less than $2\sqrt{(d+K)\tau}$, and by using a similar argument as case 1,  we have:
\begin{align}
    \widehat f^\con({\blambda^t, \bmu^t}) &\geq  \widehat f^\con(\blambda^*, \bmu^*) - 8(d+K) \sqrt{\tau}
    \label{eqn:dual-subop-case2b}
\end{align}

Putting all the cases from \eqref{eqn:dual-subop-case1}, \eqref{eqn:dual-subop-case2a} and \eqref{eqn:dual-subop-case2b} together, we have
\begin{align*}
\lefteqn{\max_{0 \leq t\leq T} \widehat f^\con({\blambda^t, \bmu^t})}\\
&\geq \widehat f^\con(\blambda^*, \bmu^*) - 4a \sqrt{d+K} \exp\left(-\frac{T}{4(d+K)^2}\right) - 4a\sqrt{(d+K)\tau} -  \tau - 8(d+K) \sqrt{\tau},
\end{align*}
which completes the proof.
\end{proof}

\subsubsection{Converting  guarantee on $\hat{f}^\con$ to  primal optimality-feasibility guarantees}
Now we can bound the primal sub-optimality using a standard technique from optimization theory \cite{lee2015faster}. 

\begin{lem}
\label{lem:dual-to-primal-1}
Denote $\widetilde \cC = \textup{conv}(\{\C[h^0], \C[h^1], \ldots, \C[h^T]\})$. We then have:
\begin{align*}
\min_{\C \in \widetilde \cC, \bphi(\C) \leq 0} \psi(\C)
    &\leq
    \min_{\C \in  \cC, \bphi(\C) \leq 0} \psi(\C)+ \nu'
\end{align*}
where $\nu' =  4a \sqrt{d+K} \exp\left(-\frac{T}{4(d+K)^2}\right) + 4a\sqrt{(d+K)\tau} + 2\tau + 8(d+K) \sqrt{\tau}$.
\end{lem}
\begin{proof}
Consider an alternative version of $f^\con$ defined as 
\[
 \widetilde f^\con(\blambda, \bmu) = \min_{\C \in \widetilde \C, \bxi \in[0,1]^d} \cL^\con(\C, \xi, \blambda,  \bmu).
\] 
And let $\widehat{\widetilde{f}}^\con$ be equal to $\widetilde f^\con$ if its argument $\blambda, \bmu$ is inside the $\ell_2$-norm ball of radius $a$ and $\bmu \geq 0$, and negative infinity otherwise.

 Clearly we have that $\widehat {\widetilde f}^\con(\blambda, \bmu) \geq \widehat f^\con(\blambda, \bmu)$. We can also show $\widehat {\widetilde f}^\con$ and $\widehat f^\con$ are close at the iterates $[\blambda^t, \bmu^t]$. If $\|[\blambda^t, \bmu^t]\|>a$ or $\bmu^t \ngeq 0$, then both sides are trivially equal to negative infinity. Let $\|[\blambda^t,\bmu^t]\| \leq a$ and $\bmu^t \geq 0$. We then have:
\begin{align*}
\widehat {\widetilde f}^\con({\blambda^t, \bmu^t}) =  {\widetilde f}^\con({\blambda^t, \bmu^t}) &\leq \cL(\C[h^t], \bxi^t, {\blambda^t}, \bmu^t) \\
&= \psi(\bxi^t) - {\blambda^t}^\top \bxi^t + {\blambda^t}^\top \C[h^t] + {\bmu^t}^\top \bphi(\bxi^t) \\
&= \min_{\bxi \in \Delta_d} \left( \psi(\bxi) - {\blambda^t}^\top \bxi +  {\bmu^t}^\top \bphi(\bxi^t) \right) + {\blambda^t}^\top \C[h^t]  \\
&\leq \min_{\bxi \in \Delta_d} \left( \psi(\bxi) - {\blambda^t}^\top \bxi +  {\bmu^t}^\top \bphi(\bxi^t) \right) + \min_{\C \in \cC} {\blambda^t}^\top \C  + a \rho\\
&= \min_{\bxi \in \Delta_d, \C \in \cC} \left( \psi(\bxi) + {\blambda^t}^\top (\C - \bxi) + {\bmu^t}^\top \bphi(\bxi)  \right) + a \rho  \\
&= f^\con ({\blambda^t}, \bmu^t) + a\rho  = \widehat f^\con ({\blambda^t}, \bmu^t) + a\rho.
\end{align*}

We further have from Lemma \ref{lem:gda-con-helper} that
\begin{align*}
\max_{\blambda \in \R^d, \bmu \in \R^K_+} \widehat {\widetilde f}^\con(\blambda, \bmu) &=
 \max_{\blambda \in \R^d, \bmu \in \R^K_+} \widetilde f^\con(\blambda, \bmu).
 \end{align*}
Applying the min-max theorem to the above gives us:
 \begin{align*}
 \max_{\blambda \in \R^d, \bmu \in \R^K_+} \widetilde f^\con(\blambda, \bmu)      
 &= \max_{\blambda \in \R^d, \bmu \in \R^K_+} \min_{\C \in \widetilde \cC, \bxi \in\Delta_d} \cL^\con(\C, \xi, \blambda, \bmu) \\
 &=  \min_{\C \in \widetilde \cC, \bxi \in\Delta_d} \max_{\blambda \in \R^d, \bmu \in \R^K_+} \cL^\con(\C, \xi, \blambda, \bmu) \\
 &= \min_{\C \in \widetilde \cC, \bphi(\C) \leq 0} \psi(\C).
\end{align*}

Recall that Algorithm \ref{alg:ellipsoid-con} is designed to find the minimum of $\psi$ over $\cC$ (subject to constraints $\bphi$). However, the exact same algorithm would also apply for $\widetilde \cC$, and hence the sequence of iterates ${\blambda^t, \bmu^t}$ also approximately maximise $\widetilde f^\con$. Let $\nu$ be as defined in Theorem \ref{thm:ellipsoid-dual-con}. Then
\allowdisplaybreaks
\begin{align*}
\max_{0 \leq t\leq T} \widehat{\widetilde f}^\con({\blambda^t, \bmu^t}) 
&\geq \max_{\blambda \in \R^d, \bmu \in \R^K_+}  \widehat{\widetilde{f}}^\con(\blambda, \bmu) - \nu  \\
 \max_{\blambda \in \R^d, \bmu \in \R^K_+} \widehat{\widetilde f}^\con(\blambda, \bmu)
 & \leq \max_{0 \leq t\leq T} \widehat{\widetilde f}^\con({\blambda^t, \bmu^t})  + \nu  \\
& \leq \max_{0 \leq t\leq T}  \widehat f^\con({\blambda^t, \bmu^t})  + a\rho + \nu  \\
& \leq \max_{\blambda \in \R^d, \bmu \in \R^K_+}  \widehat f^\con(\blambda, \bmu) + \tau + \nu  \\
 \end{align*}

We thus have that
\begin{align*}
\min_{\C \in \widetilde \cC, \bphi(\C) \leq 0} \psi(\C)
    &\leq
    \min_{\C \in  \cC, \bphi(\C) \leq 0} \psi(\C)+ \tau + \nu,
\end{align*}
%  \qedsymbol
which completes the proof.
\end{proof}

\begin{lem}
\label{lem:dual-to-primal-2}
Let $\balpha^* \in \underset{\balpha \in \Delta_{T}, \bphi(\sum_t \alpha_t\C^t)\leq 0 }{\argmin} \psi\left( \sum_{i=0}^T \alpha_{i} \C^{i} \right)$.
Then:
\begin{align*}
\psi\left( \sum_{i=0}^T \alpha^*_{i} \C[h^i] \right)
&\leq 
 \min_{\C \in  \widetilde \cC, \bphi(\C) \leq 0} \psi(\C) + 2\tau; \\
\phi_k \left( \sum_{i=0}^T \alpha^*_{i} \C[h^i] \right)
&\leq \tau,
\end{align*}
where $\widetilde \C = \textup{conv}(\{\C[h^0], \ldots, \C[h^T]\})$. 
\end{lem}
\begin{proof}
Let $\bbeta^* \in \underset{\bbeta \in \Delta_{T}, \bphi(\sum_t \beta_t\C[h^t])\leq 0}{\argmin} \psi\left( \sum_{i=0}^T \beta_{i} \C[h^i] \right)$
denote the  coefficients obtained by solving a similar minimization problem with the estimates $\C^t$ replaced with the true confusion matrices $C[h^t]$. 
First, we note that $\balpha^*$ and $\bbeta^*$ exist because $h_0$ (and in turn, $\C[h^0]=\C^0$) is strictly feasible. 
\allowdisplaybreaks
\begin{align*}
\psi\left( \sum_{i=0}^T \alpha^*_{i} \C[h^i] \right)
&= \psi\left( \sum_{i=0}^T \alpha^*_{i} \C^i + \sum_{i=0}^T \alpha^*_{i}(\C[h^i]-\C^i) \right) \\
&\leq  \psi\left( \sum_{i=0}^T \alpha^*_{i} \C^i \right) + L\rho' \sqrt{d} \\
&= \min_{\balpha \in \Delta_T} \psi\left(\sum_{i=0}^T \alpha_{i} \C^i\right) + L\rho' \sqrt{d}  \\
&\leq  \psi\left(\sum_{i=0}^T \beta^*_{i} \C^i\right) + L\rho'\sqrt{d}   \\
&=  \psi\left(\sum_{i=0}^T \beta^*_{i} \C[h^i] + \sum_{i=0}^T \beta^*_{i} (\C^i - \C[h^i]) \right) + L\rho'\sqrt{d} \\
&\leq  \psi\left(\sum_{i=0}^T \beta^*_{i} \C[h^i] \right) + 2L\rho'\sqrt{d} \\
&= \min_{\bbeta \in \Delta_T, \bphi(\sum_t \beta_t\C[h^t])\leq 0} \psi\left(\sum_{i=0}^T \beta_{i} \C[h^i] \right) + 2L\rho'\sqrt{d} \\
&= \min_{\C \in \widetilde \cC, \bphi(\C) \leq 0} \psi(\C) + 2L\rho'\sqrt{d}  \\
& \leq \min_{\C \in  \widetilde \cC, \bphi(\C) \leq 0} \psi(\C) + 2\tau,
\end{align*}
where the first and third inequality above are due to the Lipschitzness of $\psi$.

Using a similar argument as above, we get for all $k \in [K]$,
\begin{align*}
\phi_k\left( \sum_{i=0}^T \alpha^*_{i} \C[h^i] \right)
&= \phi_k\left( \sum_{i=0}^T \alpha^*_{i} \C^i + \sum_{i=0}^T \alpha^*_{i}(\C[h^i]-\C^i) \right) \\
&\leq  \phi_k\left( \sum_{i=0}^T \alpha^*_{i} \C^i \right) + L\rho' \sqrt{d} \\
&\leq 0 +  L\rho' \sqrt{d} \leq \tau,
\end{align*}
where the first inequality above is due to the Lipschitzness of $\phi$, and the second inequality is due to the property of $\balpha^*$ being chosen from a set such that the weighted combination of $\C^i$ is feasible.

We are now ready to prove Theorem \ref{thm:ellipsoid-con}.
\end{proof}
\begin{proof}[Proof of Theorem \ref{thm:ellipsoid-con}]
Let $\balpha^* \in \underset{\balpha \in \Delta_{T}, \bphi(\sum_t \alpha_t\C^t)\leq \0 }{\argmin} \psi\left( \sum_{i=0}^T \alpha_{i} \C^{i} \right).$ 
Let $\nu'$ be as in Lemma \ref{lem:dual-to-primal-1}. Putting Lemmas \ref{lem:dual-to-primal-1} and \ref{lem:dual-to-primal-2} together we get, for all $k\in[K]$,
\begin{align*}
\psi(\C[\overline h]) &=  \psi\left( \sum_{i=0}^T \alpha^*_{i} \C[h^i] \right) \\
&\leq     \min_{\C \in  \cC, \bphi(\C) \leq 0} \psi(\C)+ 2\tau + \nu'  \\
&=  \min_{\C \in  \cC, \bphi(\C) \leq 0} \psi(\C) + 4a \sqrt{d+K} \cdot \exp\left(-\frac{T}{4(d+K)^2}\right) + 4a\sqrt{(d+K)\tau} + 4\tau + 8(d+K) \sqrt{\tau} \\
&= \min_{\C \in  \cC, \bphi(\C) \leq 0} \psi(\C) + 4a \sqrt{d+K} \cdot \exp\left(-\frac{T}{4(d+K)^2}\right) + 4a\sqrt{(d+K)\tau} + 4\tau + 8(d+K) \sqrt{\tau} \\
&= \min_{\C \in  \cC, \bphi(\C) \leq 0} \psi(\C) + 4a \sqrt{\bar{d}} \cdot \exp\left(-\frac{T}{4\bar{d}^2}\right) + 4a\sqrt{\bar{d} \tau} + 4\tau + 8\bar{d} \sqrt{\tau}  \\
&= \min_{\C \in  \cC, \bphi(\C) \leq 0} \psi(\C) + 4a \sqrt{\bar{d}} \cdot \exp\left(-\frac{T}{4\bar{d}^2}\right) + (4a\sqrt{\bar{d}}+8\bar{d})\sqrt{\tau} + 4\tau.
\end{align*}

We now set $T=4\bar{d}^2 \log(\frac{\bar{d}}{\epsilon})$. For small enough $\rho$ and $\rho'$, the $4\tau$ term can be bounded by $\sqrt{\tau}$  to get an order dependence of the sub-optimality. Thus we get
\begin{align*}
\psi(\C[\overline h]) 
&\leq  \min_{\C \in  \cC, \bphi(\C) \leq 0} \psi(\C) + 4a\epsilon + (4a\sqrt{\bar{d}}+8\bar{d}+4)\sqrt{\tau} \\
&\leq \min_{\C \in  \cC, \bphi(\C) \leq 0} \psi(\C) + \cO\left(\epsilon+\bar{d}\sqrt{\tau} \right)
\end{align*}

The feasibility inequality then follows easily from Lemma \ref{lem:dual-to-primal-2}
\begin{align*}
\phi_k(\C[\overline h]) &=  \phi_k\left( \sum_{i=0}^T \alpha^*_{i} \C[h^i] \right) 
~~\leq \tau, 
 \end{align*}
 where $\bar{d}=d+K$. This completes the proof.
\end{proof}



==> con-gda-proof-backup.tex <==
\begin{thm*}[(Restated) Convergence of ConGDA algorithm]
Fix $\epsilon \in (0,1)$. 
Let $\psi, \phi_1,\ldots,\phi_K: [0,1]^d\>[0,1]$ be convex and $L$-Lipschitz  w.r.t.\ the $\ell_\infty$-norm. Let $\Omega$ in Algorithm \ref{alg:GDA-con} be a $(\rho , \rho', \delta)$-approximate LMO for sample size $N$. 
Suppose there exists $\C' \in \cC$ which is strictly feasible, i.e.\ for some $r > 0$,  such that
$\max_{k\in [K]} \phi_k(\C') \leq -r$. 
Let the space of Lagrange multipliers $\Lambda = \{\blambda\in \R^d\,|\,\|\blambda\|_1\leq 2L(1 + 1/r)\}$,
and $\Xi = \{\bmu\in \R_+^K\,|\,\|\bmu\|_1\leq 2/r\}$. 
Let $B_{\bphi} \geq \max_{\bxi \in \Delta_d} \|\bphi(\bxi)\|_2$.
%Let $B_{\bxi} \geq \max_{t\in [T]}\|\bxi^t\|_2$ and $B_{\C} \geq \max_{t\in [T]}\|\C^t\|_2$. 
Let $\bar{h}$ be a classifier returned by Algorithm \ref{alg:GDA-con} when run for $T$ iterations,
% with step-sizes $\eta = \frac{B_{\bxi}}{2L\sqrt{2T}}$
% and $\eta' = \frac{L}{(B_{\bxi} + B_{\C})\sqrt{2T}}$. 
with step-sizes $\eta = \frac{\sqrt{d}}{\bar{L}\sqrt{2T}}$
and $\eta' = \frac{\bar{L}}{(2\sqrt{d} + B_\bphi)\sqrt{2T}}$, where $\bar{L} = 4(1 + 1/r)L + 2/r$.
% with a sample $S \sim D^N$. 
 Then with probability $\geq 1 - \delta$ over draw of $S \sim D^N$, after $T = \cO(d/\epsilon^2)$ iterations:
\[
\psi(\C[\bar{h}]) \,\leq\, \min_{\C \in \cC:\, \bphi(\C) \leq \0}\,\psi(\C) \,+\,\cO\left(L(\epsilon + \rho + \rho')\right)
\]
\vspace{-5pt}
\[
\phi_k(\C[\bar{h}]) \,\leq\, \cO\left(L(\epsilon + \rho + \rho')\right), \forall k \in [K].
\]
\end{thm*}

The proof is an adaptation of the proof of convergence in \citet{Narasimhan+19_generalized} for their oracle-based optimizer (Theorem 3 in their paper), but takes into account three differences:
(i) they consider a generic objective function that is independent of $\C$, (ii) they assume that $\phi_k$s are monotonic, (iii) they perform a full optimization on $\bxi$ instead of gradient-based updates. Moreover, unlike them, we employ exponentiated gradient updates, and derive a better dependence on dimension.

We will furst find it useful to first state the following lemma, 
% which follows directly from the equivalence between the min-max Lagrangian optimization and minimizing $\psi$ under constraints (see e.g. \eqref{eq:minmax-reformulation-constrained}).
which adapts the
 proof steps from Lemmas 4 and 6 in \citet{Narasimhan+19_generalized}.
\begin{lem}
\label{lem:gda-con-helper}
%  Let $\C^*$ be a minimizer of $\psi$ over $\C \in \cC$. Let $\bxi^* =\C^*$ and let $\lambda^* = \nabla\psi(\C^*)$. Then:
%  $$
% \max_{\blambda \in \Lambda}\,\cL(\C^*,\bxi^*, \blambda)
% = \min_{\C\in\cC,\, \bxi\in\Delta_d}\,\cL(\C,\bxi, \blambda^*).
% $$ 
% Suppose 
% $\psi$ is $L$-Lipschitz w.r.t.\ the $\ell_\infty$-norm, and
% $\Lambda = \{\blambda\in \R^d\,|\,\|\blambda\|_1\leq L\}$. %
% Let $\psi, \phi_1, \ldots, \phi_K$ satisfy the assumptions in Theorem \ref{thm:gda-con}.
Let $\psi, \phi_1,\ldots,\phi_K: [0,1]^d\>[0,1]$ be convex and $L$-Lipschitz  w.r.t.\ the $\ell_\infty$-norm. 
Suppose there exists $\C' \in \cC$ which is strictly feasible, i.e.\ for some $r > 0$,  such that
$\max_{k\in [K]} \phi_k(\C') \leq -r$. 
Let $\C^* \in \underset{\C \in \cC:\, \bphi(\C) \leq \0}{\argmin}\, \psi(\C)$, and let 
$$(\blambda^*, \bmu^*) \in \underset{\blambda \in \R^d, \bmu \in \R^K_+}{\argmax}\left\{
    \min_{\C \in \cC,\,\bxi\in \Delta^d} \cL^\con(\C, \bxi, \blambda, \bmu)
    \right\}.$$
Then:
\begin{enumerate}
    \item $\displaystyle
        \psi(\C^*) = \min_{\C \in \cC,\,\bxi \in \Delta_d}\max_{\blambda \in \R^d,\, \bmu \in \R^K_+}\cL^\con(\C, \bxi, \blambda, \bmu) = \max_{\blambda \in \R^d,\, \bmu \in \R^K_+}\min_{\C \in \cC,\,\bxi \in \Delta_d}\cL^\con(\C, \bxi, \blambda, \bmu);$
    % \item $\blambda^* = \nabla\psi(\C^*) + \sum_{k=1}^K \mu^*_k \nabla\phi_k(\C^*)$
    \item $\|\bmu^*\|_1 \leq 1/r$;
    \item $\|\blambda^*\|_2 \leq \sqrt{d}L(1 + 1/r)$.
\end{enumerate}

\end{lem}
\begin{proof}
For part 1, we begin by writing out the Lagrangian from \eqref{eq:lagrangian-unc}:
\[
\cL^\con(\C, \bxi, \blambda, \bmu) 
= \psi(\bxi) + \langle \blambda, \C-\bxi \rangle + \langle \bmu, \bphi(\bxi) \rangle.
\]
Since $\cL^\con$ is convex in $\bxi$ and linear in $\blambda$ and $\bmu$, strong duality holds, and we have: % for fixed $\C^*$:
\begin{eqnarray*}
\max_{\blambda \in \R^d,\, \bmu \in \R^K_+}\min_{\C \in \cC,\,\bxi \in \Delta_d}\cL^\con(\C, \bxi, \blambda, \bmu)
 &=&
    \min_{\C \in \cC,\,\bxi \in \Delta_d}\max_{\blambda \in \R^d,\, \bmu \in \R^K_+}\cL^\con(\C, \bxi, \blambda, \bmu)\\
&=& \min_{\C \in \cC,\,\bxi \in \Delta_d:\, \bxi = \C,\, \bphi(\bxi) \leq \0}\psi(\C)\\
&=& \min_{\C \in \cC,:\, \bphi(\C) \leq \0}\,\psi(\C)\\
&=& \psi(\C^*).
\end{eqnarray*}

For part 2, recall that $C' \in \cC$ is  such that
$\max_{k\in [K]} \phi_k(\C') \leq -r$ for some $r>0$. 
It then follows from part 1 that:
\begin{eqnarray*}
\psi(\C^*) &=& 
\min_{\C \in \cC,\, \bxi \in \Delta_d}\cL^\con(\C, \bxi, \blambda^*, \bmu^*)\\
&\leq&
\cL^\con(\C', \C', \blambda^*, \bmu^*)\\
&\leq&
\psi(\C') +  \langle \bmu^*, \bphi(\C') \rangle\\
&=&
\psi(\C') - r\|\bmu^*\|_1.
\end{eqnarray*}
We thus have:
\[
\|\bmu^*\|_1 \,\leq\, (\psi(\C') - \psi(\C^*))/ r \,=\, 1/r.
\]

For part 3, 
letting $\omega(\bxi) = \psi(\bxi) + \langle \bmu^*, \bphi(\bxi) \rangle$,
we note that: %for fixed $\C^*$ and $\bmu^*$:
\begin{eqnarray}
\max_{\blambda \in \R^d}\min_{\bxi \in \Delta_d}\cL^\con(\C^*, \bxi, \blambda, \bmu^*)
&=&
\min_{\bxi \in \Delta_d}\cL^\con(\C^*, \bxi, \blambda^*, \bmu^*)
\nonumber
\\
&=&
    \min_{\bxi \in \Delta_d}
    \left\{
        \psi(\bxi) + \langle \bmu^*, \bphi(\bxi) \rangle
        - \langle \blambda^*, \bxi \rangle 
    \right\}
    + \langle \blambda^*, \C^* \rangle
    \nonumber
\\
&=& 
    \min_{\bxi \in \Delta_d}
        \left\{
            \omega(\bxi) - \langle \blambda^*, \bxi \rangle 
        \right\}
    + \langle \blambda^*, \C^* \rangle
    \nonumber
\\
&=& 
     -\omega^*(\blambda^*)
    + \langle \blambda^*, \C^* \rangle,
    \label{eq:fy-rhs}
\end{eqnarray}
where $\omega^*$ denotes the Fenchel conjugate of $\omega$. 
We similarly note that:
\begin{eqnarray}
\max_{\blambda \in \R^d}\min_{\bxi \in \Delta_d}\cL^\con(\C^*, \bxi, \blambda, \bmu^*)
&=& 
    \max_{\blambda \in \R^d}
    \left\{
    \min_{\bxi \in \Delta_d}
        \left\{
            \omega(\bxi) - \langle \blambda, \bxi \rangle 
        \right\}
    + \langle \blambda, \C^* \rangle
    \right\}
    \nonumber
\\
&=& 
\max_{\blambda \in \R^d}
    \left\{
     -\omega^*(\blambda)
    + \langle \blambda, \C^* \rangle
    \right\}
    \nonumber
    \\
&=&
\omega^{**}(\C^*)
~=~
\omega(\C^*),
    \label{eq:fy-lhs}
\end{eqnarray}
where $\omega^{**}$ denotes the second Fenchel conjugate of $\omega$. 
From \eqref{eq:fy-rhs} and \eqref{eq:fy-lhs},
its clear that:
\[
\omega(\C^*) 
\,=\,
-\omega^*(\blambda^*)
    + \langle \blambda^*, \C^* \rangle.
\]
An application of the Fenchel-Young inequality then gives us that:
\[
\lambda^* = \nabla\omega(\C^*) =
\nabla\psi(\C^*) + \sum_{k=1}^K \mu^*_k \nabla\phi_k(\C^*).
\]
We can thus bound the norm of $\blambda^*$ as:
\begin{eqnarray*}
\|\lambda^*\|_2
&\leq&
\|\nabla\psi(\C^*)\|_2
+ 
\sum_{k=1}^K|\mu_k^*|\|\nabla\phi_k(\C^*)\|_2\\
&\leq&
\|\nabla\psi(\C^*)\|_2
+ 
\|\bmu^*\|_1\,\max_{k \in K}\|\nabla\phi_k(\C^*)\|_2\\
&\leq&
\sqrt{d}\|\nabla\psi(\C^*)\|_\infty
+ 
\sqrt{d}\|\bmu^*\|_1\,\max_{k \in K}\|\nabla\phi_k(\C^*)\|_\infty\\
&\leq&
\sqrt{d}L(1 + 1/r),
\end{eqnarray*}
which follows from part 2 and the fact that $\psi$ and $\phi_k$s are Lipschitz w.r.t. the $\ell_1$-norm.
\end{proof}
% \begin{proof}
% Because $\bxi^* = \C^*$, we have:
% \begin{eqnarray*}
% \text{LHS} &=& \max_{\blambda \in \Lambda}\,\psi(\C^*) + \langle \blambda, \0\rangle ~=~ \psi(\C^*).
% \end{eqnarray*}
% \begin{eqnarray*}
% \text{RHS} &=&
% \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,  \psi(\bxi) + \langle \nabla\psi(\C^*), \C - \bxi\rangle
% \end{eqnarray*}
% \end{proof}

\begin{proof}[Proof of Theorem \ref{thm:gda-unc}]
% Let $(\C^*, \bxi^*, \blambda^*)$ be an exact saddle-point for the min-max problem in \eqref{eq:minmax-reformulation}, i.e. 
% $$
% \max_{\lambda \in \Lambda}\,\cL(\C^*,\bxi^*, \blambda)
% = \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C,\bxi, \blambda^*).
% $$ 
% Such a saddle-point exists because \eqref{eq:minmax-reformulation} forms a convex-linear min-max game. 
% We then have from Lemma 2 in \citet{Narasimhan+19_generalized} that $\C^*$ is a minimizer of $\psi$ over $\cC$, $\bxi^*=\C^*$ and $\|\blambda^*\|_1 \leq L$.
%
Pick $B_{\bxi} \geq \max_{\xi \in [0,1]^d}\|\bxi\|_2$, $B_{\C} \geq \max_{\C \in \cC}\|\C\|_2$. 
We begin by writing out the Lagrangian from \eqref{eq:lagrangian-unc}:
\[
\cL^\con(\C, \bxi, \blambda, \bmu) 
= \psi(\bxi) + \langle \blambda, \C-\bxi \rangle + \langle \bmu, \bphi(\bxi) \rangle
= 
\underbrace{\psi(\bxi) - \langle \blambda, \bxi \rangle  + \langle \bmu, \bphi(\C) \rangle}_{\cL_1(\bxi, \blambda, \bmu)} + 
\underbrace{\langle \blambda, \C \rangle}_{\cL_2(\C, \blambda)}.
\]


\textbf{Optimality.} 
To show optimality, note that $\cL_1$ is convex in $\xi$ and linear in $\blambda$ and $\bmu$, and $\cL_2$ is linear both in $\C$ and $\blambda$. Following the same steps in the proof of Theorem \ref{thm:gda-unc}, the use of a $(\rho , \rho', \delta)$-approximate LMO to compute $\C^t$ and $h^t$ at each iteration gives us with probability at least $1-\delta$ (over draw of $S$):
\begin{eqnarray}
\frac{1}{T}\sum_{t=1}^T\cL_2(\C^t, \blambda^t) &\leq&
\frac{1}{T}\sum_{t=1}^T\cL_2(\C[h^t], \blambda^t) \,+\, \|\blambda^t\|_\infty\|\C^t - \C[h^t]\|_1
\nonumber
\\
% &=&
% \frac{1}{T}\sum_{t=1}^T\langle \blambda^t, \C[h^t] \rangle \,+\, \|\blambda^t\|_\infty\|\C^t - \C[h^t]\|_1
% \nonumber
% \\
% &=&
% \|\blambda^t\|_2\frac{1}{T}\sum_{t=1}^T\left\langle \frac{\blambda^t}{\|\blambda^t\|_2}, \C[h^t] \right\rangle \,+\, \|\blambda^t\|_\infty\|\C^t - \C[h^t]\|_1
% \nonumber
% \\
% &\leq &
% \|\blambda^t\|_2\frac{1}{T}\sum_{t=1}^T\min_{\C \in \cC}\left\langle \frac{\blambda^t}{\|\blambda^t\|_2}, \C \right\rangle \,+\,
% \|\blambda^t\|_2\rho \,+\,
% \|\blambda^t\|_\infty\rho'
% \nonumber
% \\
% &=&
% \frac{1}{T}\sum_{t=1}^T\min_{\C\in\cC}\,\cL_2(\C, \blambda^t) \,+\,
% \|\blambda^t\|_2\rho \,+\, \|\blambda^t\|_\infty\rho'
% \nonumber
% \\
&\leq&
\min_{\C\in\cC}\frac{1}{T}\sum_{t=1}^T\cL_2(\C, \blambda^t) \,+\, 2\sqrt{d}L(1+1/r)(\rho + \rho').
\label{eq:gda-con-lmo}
\end{eqnarray}
% where the fourth step from the properties of the LMO in Definition \ref{defn:lmo} and the last step follows from the projection of the Lagrange multipliers onto $\Lambda$, which guarantees that $\|\blambda^t\|_\infty \leq \|\blambda^t\|_2 \leq \|\blambda^t\|_1 \leq L, \forall t$. The last three steps hold with probability at least $1-\delta$ (over draw of $S$).

Next, we apply the classical regret bound guarantee for online gradient \textit{descent} \citep{Zinkevich03,shalev2011online}, we have from the sequence of objectives $\cL_1(\cdot, \blambda^t, \bmu^t)$'s (where the optimization is over $\xi$). Note that 
$\|\nabla_\bxi \cL_1(\bxi, \blambda^t, \bmu^t)\|_2 \leq 
\|\nabla_\bxi \cL_1(\bxi, \blambda^t, \bmu^t)\|_1 \leq
\|\nabla_\bxi \psi(\bxi)\|_1 +
\|\blambda^t\|_1 + \|\bmu^t\|_1\max_k \|\nabla_\bxi \phi_k(\bxi)\|_1
\leq
L + 2L(1+1/r) + 2L/r =
(3 + 4/r)L \leq \bar{L}$. So with
$\eta = \frac{B_\bxi}{\bar{L}\sqrt{2T}}$, we have:
\begin{eqnarray}
\frac{1}{T}\sum_{t=1}^T\cL_1(\bxi^t, \blambda^t, \bmu^t)~\leq~
\min_{\bxi\in [0,1]^d}\,\sum_{t=1}^T\,\cL_1(\bxi, \blambda^t, \bmu^t) \,+\, 
% \cO\left(\frac{1}{\sqrt{T}}\right).
\frac{\sqrt{2}B_{\bxi}\bar{L}}{\sqrt{T}}.
\label{eq:gda-con-xi-regret}
\end{eqnarray}
Combining \eqref{eq:gda-con-lmo} and \eqref{eq:gda-con-xi-regret}, we have with probability at least $1-\delta$ (over draw of $S$):
\begin{eqnarray}
\lefteqn{\frac{1}{T}\sum_{t=1}^T\cL^\con(\C^t, \bxi^t, \blambda^t, \bmu^t)}
\nonumber\\
&\leq&
\min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\sum_{t=1}^T\,\cL^\con(\C, \bxi, \blambda^t, \bmu^t) \,+\, \frac{\sqrt{2}B_{\bxi}\bar{L}}{\sqrt{T}} \,+\, 2L(1+1/r)(\rho + \rho')
\nonumber
\\
&=&
\min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C, \bxi, \bar{\blambda}, \bar{\bmu}) \,+\, \frac{\sqrt{2}B_{\bxi}\bar{L}}{\sqrt{T}} \,+\, 2L(1+1/r)(\rho + \rho')
\nonumber
\\
&\leq&
\max_{\blambda \in \R^d, \bmu \in \R^K_+}\min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL^\con(\C, \bxi, {\blambda}, \bmu) \,+\, \frac{\sqrt{2}B_{\bxi}\bar{L}}{\sqrt{T}} \,+\, 2L(1+1/r)(\rho + \rho')
\nonumber\\
&=&
\min_{\C\in\cC}\left\{\max_{\blambda \in \R^d, \bmu \in \R^K_+}\,\min_{\bxi\in[0,1]^d}\,\cL^\con(\C, \bxi, {\blambda}, \bmu)\right\} \,+\, \frac{\sqrt{2}B_{\bxi}\bar{L}}{\sqrt{T}} \,+\, 2L(1+1/r)(\rho + \rho')
\nonumber\\
&=&
\min_{\C\in\cC:\, \bphi(\C) \leq \0}\psi(\C) \,+\, \frac{\sqrt{2}B_{\bxi}\bar{L}}{\sqrt{T}} \,+\, 2L(1+1/r)(\rho + \rho'),
\label{eq:gda-con-C-xi}
\end{eqnarray}
where in the second step $\bar{\blambda} = \frac{1}{T}\sum_{t=1}^T\blambda^t$ and $\bar{\bmu} = \frac{1}{T}\sum_{t=1}^T\bmu^t$ and we use the linearity of $\cL$ in $\blambda$ and $\bmu$; in the fourth step we use strong duality to interchange the max and min; and in the last step follows
from Lemma \ref{lem:gda-con-helper}.
% we use the equivalence between the min-max Lagrangian optimization and minimizing $\psi$ under constraints (see e.g. \eqref{eq:minmax-reformulation-constrained}).

Similarly, we apply the standard online gradient \textit{ascent} analysis on the sequence of losses $\cL^\con(\C^t, \bxi^t, \cdot, \cdot)$'s, where the optimization is over $\blambda$ and $\bmu$. 
Note that
$\|\nabla_{\blambda, \bmu}\, \cL^\con(\C^t, \bxi^t,\blambda^t, \bmu^t)\|_2 = \|\C^t - \bxi^t\|_2 +\|\bphi(\bxi^t)\|_2 \leq B_{\C} + B_{\bxi} + B_{\bphi}$
and $
\textstyle
\left\|
\begin{bmatrix}
\blambda\\
\bmu
\end{bmatrix}
\right\|_2 \leq 
\left\|
\begin{bmatrix}
\blambda\\
\bmu
\end{bmatrix}
\right\|_1
\leq 2L(1 + 1/r) + 2/r \leq \bar{L}
$. 
So with 
$\eta' = \frac{\bar{L}}{(B_{\bxi} + B_{\C} + B_{\bphi})\sqrt{2T}}$, we have:
\begin{eqnarray}
\lefteqn{\frac{1}{T}\sum_{t=1}^T\cL^\con(\C^t, \bxi^t, \blambda^t, \bmu^t)}
\nonumber\\
&\geq&
\max_{\blambda \in \Lambda, \, \bmu \in \Xi}\,\sum_{t=1}^T\,\cL^\con(\C^t, \bxi^t, \blambda, \bmu) \,-\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
\nonumber
\\
&\geq&
\max_{\blambda \in \Lambda, \, \bmu \in \Xi}
\left\{
\sum_{t=1}^T\,\cL^\con(\C[h^t], \bxi^t, \blambda, \bmu)
\,-\,  \|\blambda\|_\infty\|\C^t - \C[h^t]\|_1
\right\}
\,-\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
\nonumber
\\
&\geq&
\max_{\blambda \in \Lambda, \, \bmu \in \Xi}\,\sum_{t=1}^T\,\cL(\C[h^t], \bxi^t,\blambda,\bmu) 
\,-\,  L(1+1/r)\rho'
\,-\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
\nonumber
\\
&\geq&
\max_{\blambda \in \Lambda, \, \bmu \in \Xi}\,\cL^\con(\C[\bar{h}], \bar{\bxi},\blambda, \bmu) 
\,-\,  2L(1+1/r)\rho'
\,-\,  \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
\nonumber\\
% &\geq&
% \max_{\blambda \in \Lambda}\,\cL^\con(\C[\bar{h}], \bar{\bxi},\blambda, \0) 
% \,-\,  L\rho'
% \,-\,  \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
% \nonumber\\
&=&
\max_{\blambda \in \Lambda}\left\{
\psi(\bar{\bxi}) + \langle \blambda, \C[\bar{h}]-\bar{\bxi} \rangle \right\}
\,+\, \max_{\bmu \in \Xi}\, \langle \bmu, \bphi(\bar{\bxi}) \rangle
\,-\,  2L(1+1/r)\rho'
\,-\,  \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
\label{eq:gda-con-lambda-common}\\
&\geq&
\min_{\bxi\in [0,1]^d}\left\{
\max_{\blambda \in \Lambda}\,\left\{
\psi(\bxi) + \langle \blambda, \C[\bar{h}]-\bxi \rangle \right\}
\,+\, \max_{\bmu \in \Xi}\, \langle \bmu, \bphi(\bxi) \rangle
\right\}
\,-\,  2L(1+1/r)\rho'
 \,-\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
\nonumber
% \\
% &=&
% \psi(\C[\bar{h}])
% \,+\, \max_{\bmu \in \Xi}\, \langle \bmu, \bphi(\bar{\bxi}) \rangle
% \,-\,  L\rho'
% \,-\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}},
% 
\\
&\geq&
\min_{\bxi\in [0,1]^d}\left\{
\max_{\blambda \in \Lambda}\,\left\{
\psi(\bxi) + \langle \blambda, \C[\bar{h}]-\bxi \rangle \right\}
\,+\,  \langle \0, \bphi(\bxi) \rangle
\right\}
\,-\,  2L(1+1/r)\rho'
 \,-\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
\nonumber
\\
&=&
\psi(\C[\bar{h}])
\,-\,  2L(1+1/r)\rho'
\,-\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}},
\label{eq:gda-con-lambda-opt}
\end{eqnarray}
where
in the third step, we use the fact that for any $\lambda \in \Lambda$,  $\|\blambda\|_\infty \leq \|\blambda\|_1 \leq L$, and the property of the LMO. 
In the fourth step, we use 
$\C[\bar{h}] = \frac{1}{T}\sum_{t=1}^T \C[h^t]$ and $\bar{\bxi} = \frac{1}{T}\sum_{t=1}^T \bxi^t$, and use the linearity of $\cL$ in $\C$, and convexity of $\cL$ in $\bxi$ and Jensen's inequality. In the last step, we apply Lemma \ref{lem:gda-unc-helper}. 
The last six steps hold with probability at least $1-\delta$.

Combining \eqref{eq:gda-con-C-xi} and \eqref{eq:gda-con-lambda-opt},
we get with probability at least $1-\delta$ (over draw of $S$), for any $\bmu' \in \Xi$
\begin{eqnarray*}
\psi(\C[\bar{h}])  \leq \min_{\C \in \cC:\, \bphi(\C) \leq \0}\,\psi(\C)
\,+\, \frac{\sqrt{2}\bar{L}(3B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
\,+\, 2L(1+1/r)(\rho + 2\rho').
% \label{eq:gda-con-opt}
\end{eqnarray*}
Setting
$T=((\sqrt{d}+B_\bphi)/\epsilon)^2$ and $B_\bxi = B_\C = \sqrt{d}$
completes the proof of optimality.


\textbf{Feasibility.} 
Let $\C^*, \blambda^*, \bmu^*$ be as defined in Lemma \ref{lem:gda-con-helper}. 
To show feasibility, combining \eqref{eq:gda-con-C-xi} and \eqref{eq:gda-con-lambda-common}, and
interchanging the min and max, we get:
\begin{equation}
\max_{\blambda \in \Lambda, \bmu \in \Xi}\left\{
\psi(\bxi) + \langle \blambda, \C[\bar{h}]-\bar{\bxi} \rangle
\,+\, \langle \bmu, \bphi(\bar{\bxi}) \rangle
\right\}
\,\leq\,
\psi(\C^*) 
\,+\,  2L(1+1/r)\rho'
 \,+\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}.
 \label{eq:gda-con-feas}
\end{equation}
Let $k' \in \argmax_{k\in[K]}\, \phi_k(\C[\bar{h}])$ denote the index of the most-violated among the $K$ constraints $\phi_1(\C[\bar{h}]), \ldots, \phi_K(\C[\bar{h}])$. Also let $\blambda' = \blambda^*$
and $\mu'_{k'} =  \mu^*_{k'} + \frac{1}{2r}$ and $\mu'_{k} =  \mu^*_{k}, \forall k \ne k'$. 
Note that
$\blambda' \in \Lambda$ and
$\bmu' \in \Xi$. 
Substituting $(\mu', \lambda')$ into the LHS of \eqref{eq:gda-con-feas}, we have:
\begin{equation*}
\psi(\bar{\bxi}) + \langle \blambda^*, \C[\bar{h}]-\bar{\bxi} \rangle
\,+\, \langle \bmu^*, \bphi(\bxi) \rangle
\,+\, \frac{1}{2r}\max_{k}\,\phi_k(\bar{\bxi})
\,\leq\,
\psi(\C^*) 
\,+\,  2L(1+1/r)\rho'
 \,+\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}},
\end{equation*}
and we further get:
\begin{eqnarray*}
\lefteqn{
\min_{\C\in \cC,\, \bxi\in [0,1]^d}\,\left\{
\psi(\bxi) + \langle \blambda^*, \C-\bxi \rangle
\,+\, \langle \bmu^*, \bphi(\bxi) \rangle
\right\}
\,+\, \frac{1}{2r}\max_{k}\,\phi_k(\bar{\bxi})}
\\
&\leq&
\psi(\C^*) 
\,+\,  2L(1+1/r)\rho'
 \,+\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}.
\end{eqnarray*}
Applying Lemma \ref{lem:gda-con-helper}, 
\begin{equation*}
\psi(\C^*) 
\,+\, \frac{1}{2r}\max_{k}\,\phi_k(\C[\bar{h}])
\,\leq\,
\psi(\C^*) 
\,+\,  2L(1+1/r)\rho'
 \,+\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}},
\end{equation*}
giving us for all $k$:
\begin{equation}
\phi_k(\bar{\bxi})
\,\leq\,
2r
\left(
2L(1+1/r)\rho'
 \,+\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}\right),
 \label{eq:gda-con-feas-1}
\end{equation}
from Lemma \ref{lem:gda-con-helper}.

Next let $j' \in \argmax_{j\in[d]}\, \left|\C_j[\bar{h}] - \bar{\xi}_j\right|$, and set
$\bmu' = \bmu^*$
and $$\lambda'_{j'} =  \lambda^*_{j'} + \frac{1}{2L(1+1/r)}\sign(\C_{j'}[\bar{h}] - \bar{\xi}_{j'})$$ and $\lambda'_{j} =  \lambda^*_{j}, \forall j \ne j'$. Substituting $(\mu', \lambda')$ into the LHS of \eqref{eq:gda-con-feas}, we have:
\begin{eqnarray*}
\lefteqn{
\psi(\bar{\bxi}) + \langle \blambda^*, \C[\bar{h}]-\bar{\bxi} \rangle
\,+\, \langle \bmu^*, \bphi(\bxi) \rangle
\,+\, \frac{1}{2L(1+1/r)}\max_{j}\,\left|\C_j[\bar{h}] - \bar{\xi}_j\right|}\\
&\leq&
\psi(\C^*) 
\,+\,  2L(1+1/r)\rho'
 \,+\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}},\hspace{5cm}
\end{eqnarray*}
and again applying Lemma \ref{lem:gda-con-helper},
we get
\begin{eqnarray}
{\max_{j}\,\left|\C_j[\bar{h}] - \bar{\xi}_j\right|}
&\leq&
\frac{2}{L(1+1/r)}\left(2L(1+1/r)\rho'
 \,+\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}\right).
 \label{eq:gda-con-feas-2}
\end{eqnarray}
Combining \eqref{eq:gda-con-feas-1} and \eqref{eq:gda-con-feas-2}, and using the Lipschitz property of $\phi_k$, we get for all $k$:
\begin{eqnarray*}
\phi_k(\C[\bar{h}])
&\leq&
L\max_{j}\,\left|\C_j[\bar{h}] - \bar{\xi}_j\right|
\,+\,
\frac{2}{L(1+1/r)}
\left(
L\rho'
 \,+\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
 \right)\\
 &\leq&
\frac{2r(2+r)}{1+r}
\left(
2L(1+1/r)\rho'
 \,+\, \frac{\sqrt{2}\bar{L}(B_{\bxi} + B_{\C} + B_{\bphi})}{\sqrt{T}}
 \right).
\end{eqnarray*}
\todohari{Verify first step. In \citet{Narasimhan+19_generalized}, this is an elaborate lemma (Lem 5).} 
Setting
$T=((\sqrt{d}+B_\bphi)/\epsilon)^2$ and $B_\bxi = B_\C = \sqrt{d}$
completes the proof of feasibility.
\end{proof}
%%%%%%%%%%%

==> gda-proof-backup.tex <==
\begin{thm*}[(Restated) Convergence of GDA algorithm]
Fix $\epsilon \in (0,1)$. 
Let $\psi: [0,1]^d\>[0,1]$ be convex and $L$-Lipschitz w.r.t.\ the $\ell_\infty$-norm. Let $\Omega$ in Algorithm \ref{alg:GDA} be a $(\rho , \rho', \delta)$-approximate LMO for sample size $N$. Let the space of Lagrange multipliers $\Lambda = \{\blambda\in \R^d\,|\,\|\blambda\|_1\leq L\}$. 
%Let $B_{\bxi} \geq \max_{t\in [T]}\|\bxi^t\|_2$ and $B_{\C} \geq \max_{t\in [T]}\|\C^t\|_2$. 
Let $\bar{h}$ be a classifier returned by Algorithm \ref{alg:GDA} when run for $T$ iterations,
% with step-sizes $\eta = \frac{B_{\bxi}}{2L\sqrt{2T}}$
% and $\eta' = \frac{L}{(B_{\bxi} + B_{\C})\sqrt{2T}}$. 
with step-sizes $\eta = \frac{\sqrt{d}}{2L\sqrt{2T}}$
and $\eta' = \frac{L}{2\sqrt{2dT}}$.  
% with a sample $S \sim D^N$. 
 Then with probability $\geq 1 - \delta$ over draw of $S \sim D^N$, after $T = \cO(d/\epsilon^2)$ iterations:
\[
\psi(\C[\bar{h}]) \,\leq\, \min_{\C \in \cC}\,\psi(\C) \,+\,\cO\left(L(\epsilon + \rho + \rho')\right).
\]
\end{thm*}

The proof is an adaptation of the proof of convergence in \citet{Narasimhan+19_generalized} for their oracle-based optimizer (Theorem 1 in their paper). 
We will find it useful to first state the following lemma, which follows the
same proof steps as Lemma 2 in \citet{Narasimhan+19_generalized}.
\begin{lem}
\label{lem:gda-unc-helper}
%  Let $\C^*$ be a minimizer of $\psi$ over $\C \in \cC$. Let $\bxi^* =\C^*$ and let $\lambda^* = \nabla\psi(\C^*)$. Then:
%  $$
% \max_{\blambda \in \Lambda}\,\cL(\C^*,\bxi^*, \blambda)
% = \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C,\bxi, \blambda^*).
% $$ 
Suppose 
$\psi$ is $L$-Lipschitz w.r.t.\ the $\ell_\infty$-norm, and
$\Lambda = \{\blambda\in \R^d\,|\,\|\blambda\|_1\leq L\}$. 
Then for any $\C' \in [0,1]^d$:
\[
\psi(\C') = \max_{\blambda \in \Lambda}\min_{\bxi \in [0,1]^d}\cL(\C', \bxi, \blambda) = \min_{\bxi \in [0,1]^d}\max_{\blambda \in \Lambda}\cL(\C', \bxi, \blambda).
\]
\end{lem}
% \begin{proof}
% Because $\bxi^* = \C^*$, we have:
% \begin{eqnarray*}
% \text{LHS} &=& \max_{\blambda \in \Lambda}\,\psi(\C^*) + \langle \blambda, \0\rangle ~=~ \psi(\C^*).
% \end{eqnarray*}
% \begin{eqnarray*}
% \text{RHS} &=&
% \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,  \psi(\bxi) + \langle \nabla\psi(\C^*), \C - \bxi\rangle
% \end{eqnarray*}
% \end{proof}

\begin{proof}[of Theorem \ref{thm:gda-unc}]
% Let $(\C^*, \bxi^*, \blambda^*)$ be an exact saddle-point for the min-max problem in \eqref{eq:minmax-reformulation}, i.e. 
% $$
% \max_{\lambda \in \Lambda}\,\cL(\C^*,\bxi^*, \blambda)
% = \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C,\bxi, \blambda^*).
% $$ 
% Such a saddle-point exists because \eqref{eq:minmax-reformulation} forms a convex-linear min-max game. 
% We then have from Lemma 2 in \citet{Narasimhan+19_generalized} that $\C^*$ is a minimizer of $\psi$ over $\cC$, $\bxi^*=\C^*$ and $\|\blambda^*\|_1 \leq L$.
%
Pick $B_{\bxi} \geq \max_{\xi \in [0,1]^d}\|\bxi\|_2$ and $B_{\C} \geq \max_{\C \in \cC}\|\C\|_2$. 
We begin by writing out the Lagrangian from \eqref{eq:lagrangian-unc}:
\[
\cL(\C, \bxi, \blambda) 
= \psi(\bxi) + \langle \blambda, \C-\bxi \rangle
= 
\underbrace{\psi(\bxi) - \langle \blambda, \bxi \rangle}_{\cL_1(\bxi, \blambda)} + 
\underbrace{\langle \blambda, \C \rangle}_{\cL_2(\C, \blambda)}.
\]
Note that $\cL_1$ is convex in $\xi$ and linear in $\blambda$, and $\cL_2$ is linear in both $\C$ and $\blambda$. The use of a $(\rho , \rho', \delta)$-approximate LMO to compute $\C^t$ and $h^t$ at each iteration gives us: % with probability at least $1-\delta$:
\begin{eqnarray}
\frac{1}{T}\sum_{t=1}^T\cL_2(\C^t, \blambda^t) &\leq&
\frac{1}{T}\sum_{t=1}^T\cL_2(\C[h^t], \blambda^t) \,+\, \|\blambda^t\|_\infty\|\C^t - \C[h^t]\|_1
\nonumber
\\
&=&
\frac{1}{T}\sum_{t=1}^T\langle \blambda^t, \C[h^t] \rangle \,+\, \|\blambda^t\|_\infty\|\C^t - \C[h^t]\|_1
\nonumber
\\
&=&
\|\blambda^t\|_\infty\frac{1}{T}\sum_{t=1}^T\left\langle \frac{\blambda^t}{\|\blambda^t\|_\infty}, \C[h^t] \right\rangle \,+\, \|\blambda^t\|_\infty\|\C^t - \C[h^t]\|_1
\nonumber
\\
&\leq &
\|\blambda^t\|_\infty\frac{1}{T}\sum_{t=1}^T\min_{\C \in \cC}\left\langle \frac{\blambda^t}{\|\blambda^t\|_\infty}, \C \right\rangle \,+\,
\|\blambda^t\|_\infty\rho \,+\,
\|\blambda^t\|_\infty\rho'
\nonumber
\\
&=&
\frac{1}{T}\sum_{t=1}^T\min_{\C\in\cC}\,\cL_2(\C, \blambda^t) \,+\,
\|\blambda^t\|_2(\rho +\rho')
\nonumber
\\
&\leq&
\min_{\C\in\cC}\frac{1}{T}\sum_{t=1}^T\cL_2(\C, \blambda^t) \,+\, L(\rho + \rho'),
\label{eq:gda-unc-lmo}
\end{eqnarray}
where the fourth step from the properties of the LMO in Definition \ref{defn:lmo} and the last step follows from the projection of the Lagrange multipliers onto $\Lambda$, which guarantees that $\|\blambda^t\|_\infty \leq \|\blambda^t\|_2 \leq \|\blambda^t\|_1 \leq L, \forall t$. The last three steps hold with probability at least $1-\delta$ (over draw of $S$).

Next, we apply the classical regret bound guarantee for online gradient \textit{descent} \citep{Zinkevich03,shalev2011online}, we have from the sequence of objectives $\cL_1(\cdot, \blambda^t)$'s (where the optimization is over $\xi$). Because 
$\|\nabla_\bxi \cL_1(\bxi, \blambda)\|_2 \leq 2L$, with
$\eta = \frac{B_\bxi}{2L\sqrt{2T}}$, we have:
\begin{eqnarray}
\frac{1}{T}\sum_{t=1}^T\cL_1(\bxi^t, \blambda^t)~\leq~
\min_{\bxi\in [0,1]^d}\,\sum_{t=1}^T\,\cL_1(\bxi, \blambda^t) \,+\, 
% \cO\left(\frac{1}{\sqrt{T}}\right).
\frac{2\sqrt{2}B_{\bxi}L}{\sqrt{T}}.
\label{eq:gda-unc-xi-regret}
\end{eqnarray}
Combining \eqref{eq:gda-unc-lmo} and \eqref{eq:gda-unc-xi-regret}, we have with probability at least $1-\delta$ (over draw of $S$):
\begin{eqnarray}
\frac{1}{T}\sum_{t=1}^T\cL(\C^t, \bxi^t, \blambda^t)&\leq&
\min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\sum_{t=1}^T\,\cL(\C, \bxi, \blambda^t) \,+\, \frac{2\sqrt{2}B_{\bxi}L}{\sqrt{T}} \,+\, L\rho \,+\, L\rho'
\nonumber
\\
&=&
\min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C, \bxi, \bar{\blambda}) \,+\, \frac{2\sqrt{2}B_{\bxi}L}{\sqrt{T}} \,+\, L\rho \,+\, L\rho'
\nonumber
\\
&\leq&
\max_{\blambda \in \Lambda}\min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C, \bxi, {\blambda}) \,+\, \frac{2\sqrt{2}B_{\bxi}L}{\sqrt{T}} \,+\, L\rho \,+\, L\rho'
\nonumber\\
&=&
\min_{\C\in\cC}\left\{\max_{\blambda \in \Lambda}\,\min_{\bxi\in[0,1]^d}\,\cL(\C, \bxi, {\blambda})\right\} \,+\, \frac{2\sqrt{2}B_{\bxi}L}{\sqrt{T}} \,+\, L\rho \,+\, L\rho'
\nonumber\\
&=&
\min_{\C\in\cC}\psi(\C) \,+\, \frac{2\sqrt{2}B_{\bxi}L}{\sqrt{T}} \,+\, L\rho \,+\, L\rho'
\nonumber\\
&=&
\psi(\C^*) \,+\, \frac{2\sqrt{2}B_{\bxi}L}{\sqrt{T}} \,+\, L\rho \,+\, L\rho',
\label{eq:gda-unc-C-xi}
\end{eqnarray}
where in the second step $\bar{\blambda} = \frac{1}{T}\sum_{t=1}^T\blambda^t$ and we use the linearity of $\cL$ in $\blambda$; in the fourth step we use strong duality to interchange the max and min; and in the last step we apply Lemma \ref{lem:gda-unc-helper}.

Similarly, we apply the standard online gradient \textit{ascent} analysis on the sequence of losses $\cL(\C^t, \bxi^t, \cdot)$'s, where the optimization is over $\blambda$. Because $\|\nabla_{\blambda} \cL(\C^t, \bxi^t,\blambda^t)\|_2 = \|\C^t - \bxi^t\|_2 \leq B_{\C} + B_{\bxi}$, with $\eta' = \frac{L}{(B_{\bxi} + B_{\C})\sqrt{2T}}$, we have:
\begin{eqnarray}
\frac{1}{T}\sum_{t=1}^T\cL(\C^t, \bxi^t, \blambda^t) &\geq&
\max_{\blambda \in \Lambda}\,\sum_{t=1}^T\,\cL(\C^t, \bxi^t,\blambda) \,-\, \frac{\sqrt{2}L(B_{\bxi} + B_{\C})}{\sqrt{T}}
\nonumber
\\
&\geq&
\max_{\blambda \in \Lambda}
\left\{
\sum_{t=1}^T\,\cL(\C[h^t], \bxi^t,\blambda) 
\,-\,  \|\blambda\|_\infty\|\C^t - \C[h^t]\|_1
\right\}
\,-\, \frac{\sqrt{2}L(B_{\bxi} + B_{\C})}{\sqrt{T}}
\nonumber
\\
&\geq&
\max_{\blambda \in \Lambda}\,
\sum_{t=1}^T\,\cL(\C[h^t], \bxi^t,\blambda) 
\,-\,  L\rho'
\,-\, \frac{\sqrt{2}L(B_{\bxi} + B_{\C})}{\sqrt{T}}
\nonumber
\\
&\geq&
\max_{\blambda \in \Lambda}\,\cL(\C[\bar{h}], \bar{\bxi},\blambda) 
\,-\,  L\rho'
\,-\, \frac{\sqrt{2}L(B_{\bxi} + B_{\C})}{\sqrt{T}}
\nonumber\\
&\geq&
\min_{\bxi\in [0,1]^d}\,\max_{\blambda \in \Lambda}\,\cL(\C[\bar{h}], {\bxi},\blambda)
\,-\,  L\rho'
 \,-\, \frac{\sqrt{2}L(B_{\bxi} + B_{\C})}{\sqrt{T}}
\nonumber
\\
&=&
\psi(\C[\bar{h}])
\,-\,  L\rho'
\,-\, \frac{\sqrt{2}L(B_{\bxi} + B_{\C})}{\sqrt{T}},
\label{eq:gda-unc-lambda}
\end{eqnarray}
where
in the third step, we use the fact that for any $\lambda \in \Lambda$,  $\|\blambda\|_\infty \leq \|\blambda\|_1 \leq L$, and the property of the LMO. 
In the fourth step, we use 
$\C[\bar{h}] = \frac{1}{T}\sum_{t=1}^T \C[h^t]$ and $\bar{\bxi} = \frac{1}{T}\sum_{t=1}^T \bxi^t$, and use the linearity of $\cL$ in $\C$, and convexity of $\cL$ in $\bxi$ and Jensen's inequality. In the fourth step, we apply Lemma \ref{lem:gda-unc-helper}. The last four steps hold with probability at least $1-\delta$.

Combining \eqref{eq:gda-unc-C-xi} and \eqref{eq:gda-unc-lambda}, we get with probability at least $1-\delta$ (over draw of $S$).
\begin{eqnarray*}
\psi(\C[\bar{h}]) \leq \psi(\C^*) \,+\, \frac{\sqrt{2}L(3B_{\bxi} + B_{\C})}{\sqrt{T}} \,+\, L\rho \,+\, 2L\rho'.
\end{eqnarray*}
Setting $T=1/\epsilon^2$ and $B_\bxi = B_\C = \sqrt{d}$ completes the proof.
%%%
% \begin{eqnarray}
% \max_{\blambda \in \Lambda}\,\cL(\bar{\C}, \bar{\bxi},\blambda) 
% &\leq&
% \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C, \bxi, \bar{\blambda}) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, L\rho \,+\, L\rho',
% \label{eq:gda-unc-combined}
% \end{eqnarray}
% which shows that $(\bar{\C}, \bar{\bxi}, \bar{\blambda})$ is an approximate saddle-point solution for the min-max problem in \eqref{eq:minmax-reformulation}.


% Now to complete our proof, we lower bound the LHS in \eqref{eq:gda-unc-combined} by plugging $\blambda = \0$ and upper bound the RHS of \eqref{eq:gda-unc-combined} by plugging in $\C = \bxi = \C^*$, giving us:
% \begin{eqnarray}
% \psi(\bar{\bxi})
% &\leq&
% \psi(\C^*) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, L\rho \,+\, L\rho'.
% \label{eq:gda-unc-final-1}
% \end{eqnarray}
% Next, let $k \in \argmax_{j \in [d]} |\bar{C}_j - \bar{\xi}_j|$ be an index where the slack vector $\bxi$ differs most from the confusion matrix $\bar{\C}$,
% and let $\blambda' \in \R^d$ be such that 
% $\lambda'_j = \lambda^*_j, \forall j \ne k$ and $\lambda'_k = \lambda^*_k + L\sign(\bar{C}_j - \bar{\xi}_j)$. Note that because $\|\blambda^*\|_1 \leq L$, $\|\blambda'\|_1 \leq 2L$ and therefore $\blambda' \in \Lambda$. Lower bounding the the LHS in \eqref{eq:gda-unc-combined} by plugging $\blambda = \blambda'$ and upper bounding the RHS of \eqref{eq:gda-unc-combined} by plugging in $\C = \bxi = \C^*$, we get:
% \begin{eqnarray*}
% \psi(\bar{\bxi}) \,+\, \langle \blambda^*, \bar{\C} - \bar{\bxi} \rangle \,+\, L|\bar{C}_k - \bar{\xi}_k|
% &\leq&
% \psi(\C^*) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, L\rho \,+\, L\rho',
% \end{eqnarray*}
% which further gives us:
% \begin{eqnarray*}
% \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\left\{ \psi({\bxi}) \,+\, \langle \blambda^*, {\C} - {\bxi} \rangle
% \right\} \,+\, L|\bar{C}_k - \bar{\xi}_k|
% &\leq&
% \psi(\C^*) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, L\rho \,+\, L\rho'
% \end{eqnarray*}
% or
% \begin{eqnarray*}
% \psi(\C^*) \,+\, L|\bar{C}_k - \bar{\xi}_k|
% &\leq&
% \psi(\C^*) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, L\rho \,+\, L\rho'
% \end{eqnarray*}
% or
% \begin{eqnarray}
% \max_{j \in [d]}|\bar{C}_j - \bar{\xi}_j|
% &\leq&
% \cO\left(\frac{1}{L\sqrt{T}}\right) \,+\, \frac{\rho}{L} \,+\, 2\rho'.
% \label{eq:gda-unc-final-2}
% \end{eqnarray}
% Substituting from \eqref{eq:gda-unc-final-2} into \eqref{eq:gda-unc-final-1} and using the fact that $\psi$ is $L$-Lipschitz w.r.t.\ the $\ell_1$-norm, we finally have:
% \begin{eqnarray*}
% \psi(\bar{\C})
% &\leq&
% \psi(\C^*) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, 2\rho \,+\, 4L\rho',
% \end{eqnarray*}
% which completes the proof.
\end{proof}


==> gda-proof-exp.tex <==
\begin{thm*}[(Restated) Convergence of GDA algorithm]
Fix $\epsilon \in (0,1)$. 
Let $\psi: [0,1]^d\>[0,1]$ be convex and $L$-Lipschitz w.r.t.\ the $\ell_1$-norm. Let $\Omega$ in Algorithm \ref{alg:GDA} be a $(\rho , \rho', \delta)$-approximate LMO for sample size $N$. 
%Let $B_{\bxi} \geq \max_{t\in [T]}\|\bxi^t\|_2$ and $B_{\C} \geq \max_{t\in [T]}\|\C^t\|_2$. 
Let $\bar{h}$ be a classifier returned by Algorithm \ref{alg:GDA} when run for $T$ iterations,
% with step-sizes $\eta = \frac{B_{\bxi}}{2L\sqrt{2T}}$
% and $\eta' = \frac{L}{(B_{\bxi} + B_{\C})\sqrt{2T}}$. 
with step-sizes $\eta = \frac{1}{2L}\sqrt{\frac{\log(d)}{T}}$
and $\eta' = \frac{1}{L}\sqrt{\frac{\log(d)}{T}}$. 
% with a sample $S \sim D^N$. 
 Then with probability $\geq 1 - \delta$ over draw of $S \sim D^N$, after $T = \cO(\log(d)/\epsilon^2)$ iterations:
\[
\psi(\C[\bar{h}]) \,\leq\, \min_{\C \in \cC}\,\psi(\C) \,+\,\cO\left(L(\epsilon + \rho + \rho')\right).
\]
\end{thm*}

The proof is an adaptation of the proof of convergence in \citet{Narasimhan+19_generalized} for their oracle-based optimizer (Theorem 1 in their paper), with one difference being that we use exponentiated gradient updates for $\bxi$ and $\blambda$, whereas they use ``full optimization'' updates for $\bxi$ and standard gradient updates for $\blambda$. 
We will find it useful to first state the following lemma, which follows the
same proof steps as Lemma 2 in \citet{Narasimhan+19_generalized}.
\begin{lem}
\label{lem:gda-unc-helper}
%  Let $\C^*$ be a minimizer of $\psi$ over $\C \in \cC$. Let $\bxi^* =\C^*$ and let $\lambda^* = \nabla\psi(\C^*)$. Then:
%  $$
% \max_{\blambda \in \Lambda}\,\cL(\C^*,\bxi^*, \blambda)
% = \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C,\bxi, \blambda^*).
% $$ 
Suppose 
$\psi$ is $L$-Lipschitz w.r.t.\ the $\ell_1$-norm, and
$\Lambda = \{\blambda\in \R^d\,|\,\|\blambda\|_1\leq Ld\}$. 
Then for any $\C' \in [0,1]^d$:
\[
\psi(\C') = \max_{\blambda \in \Lambda}\min_{\bxi \in \Delta_d}\cL(\C', \bxi, \blambda) = \min_{\bxi \in \Delta_d}\max_{\blambda \in \Lambda}\cL(\C', \bxi, \blambda).
\]
\end{lem}
% \begin{proof}
% Because $\bxi^* = \C^*$, we have:
% \begin{eqnarray*}
% \text{LHS} &=& \max_{\blambda \in \Lambda}\,\psi(\C^*) + \langle \blambda, \0\rangle ~=~ \psi(\C^*).
% \end{eqnarray*}
% \begin{eqnarray*}
% \text{RHS} &=&
% \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,  \psi(\bxi) + \langle \nabla\psi(\C^*), \C - \bxi\rangle
% \end{eqnarray*}
% \end{proof}

\begin{proof}[Proof of Theorem \ref{thm:gda-unc}]
% Let $(\C^*, \bxi^*, \blambda^*)$ be an exact saddle-point for the min-max problem in \eqref{eq:minmax-reformulation}, i.e. 
% $$
% \max_{\lambda \in \Lambda}\,\cL(\C^*,\bxi^*, \blambda)
% = \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C,\bxi, \blambda^*).
% $$ 
% Such a saddle-point exists because \eqref{eq:minmax-reformulation} forms a convex-linear min-max game. 
% We then have from Lemma 2 in \citet{Narasimhan+19_generalized} that $\C^*$ is a minimizer of $\psi$ over $\cC$, $\bxi^*=\C^*$ and $\|\blambda^*\|_1 \leq L$.
%
% Pick $B_{\bxi} \geq \max_{\xi \in [0,1]^d}\|\bxi\|_2$ and $B_{\C} \geq \max_{\C \in \cC}\|\C\|_2$. 
We begin by writing out the Lagrangian from \eqref{eq:lagrangian-unc}:
\[
\cL(\C, \bxi, \blambda) 
= \psi(\bxi) + \langle \blambda, \C-\bxi \rangle
= 
\underbrace{\psi(\bxi) - \langle \blambda, \bxi \rangle}_{\cL_1(\bxi, \blambda)} + 
\underbrace{\langle \blambda, \C \rangle}_{\cL_2(\C, \blambda)}.
\]
Note that $\cL_1$ is convex in $\xi$ and linear in $\blambda$, and $\cL_2$ is linear in both $\C$ and $\blambda$. 
Also note that because of the form of the exponentiated gradient update on the Lagrange multipliers $\blambda$, we have that $\|\blambda^t\|_1 \leq Ld, \forall t \in [T]$.

The use of a $(\rho , \rho', \delta)$-approximate LMO to compute $\C^t$ and $h^t$ at each iteration gives us: % with probability at least $1-\delta$:
\begin{eqnarray}
\frac{1}{T}\sum_{t=1}^T\cL_2(\C^t, \blambda^t) &\leq&
\frac{1}{T}\sum_{t=1}^T\cL_2(\C[h^t], \blambda^t) \,+\, \|\blambda^t\|_1\|\C^t - \C[h^t]\|_\infty
\nonumber
\\
&=&
\frac{1}{T}\sum_{t=1}^T\langle \blambda^t, \C[h^t] \rangle \,+\, \|\blambda^t\|_1\|\C^t - \C[h^t]\|_\infty
\nonumber
\\
&=&
\|\blambda^t\|_\infty\frac{1}{T}\sum_{t=1}^T\left\langle \frac{\blambda^t}{\|\blambda^t\|_\infty}, \C[h^t] \right\rangle \,+\, \|\blambda^t\|_1\|\C^t - \C[h^t]\|_\infty
\nonumber
\\
&\leq &
\|\blambda^t\|_\infty\frac{1}{T}\sum_{t=1}^T\min_{\C \in \cC}\left\langle \frac{\blambda^t}{\|\blambda^t\|_\infty}, \C \right\rangle \,+\,
\|\blambda^t\|_\infty\rho \,+\,
\|\blambda^t\|_1\rho'
\nonumber
\\
&=&
\frac{1}{T}\sum_{t=1}^T\min_{\C\in\cC}\,\cL_2(\C, \blambda^t) \,+\,
\|\blambda^t\|_\infty\rho \,+\,
\|\blambda^t\|_1\rho'
\nonumber
\\
&\leq&
\min_{\C\in\cC}\frac{1}{T}\sum_{t=1}^T\cL_2(\C, \blambda^t) \,+\, L(\rho + d\rho'),
\label{eq:gda-unc-lmo}
\end{eqnarray}
where the fourth step from the properties of the LMO in Definition \ref{defn:lmo} and the last step follows from  $\|\blambda^t\|_\infty \leq L$ and  $\|\blambda^t\|_1 \leq dL, \forall t$. The last three steps hold with probability at least $1-\delta$ (over draw of $S$).

Next, we apply the classical regret bound guarantee for exponentiated gradient \textit{descent} \citep{kivinen1997exponentiated,shalev2011online}, we have from the sequence of objectives $\cL_1(\cdot, \blambda^t)$'s (where the optimization is over $\xi$). Because 
$\|\nabla_\bxi \cL_1(\bxi, \blambda^t)\|_\infty \leq \|\nabla\psi(\bxi)\|_\infty + \|\blambda^t\|_\infty \leq 2L$, with
$\eta = \frac{1}{2L}\sqrt{\frac{\log(d)}{T}}$, we have:
\begin{eqnarray}
\frac{1}{T}\sum_{t=1}^T\cL_1(\bxi^t, \blambda^t)~\leq~
\min_{\bxi\in [0,1]^d}\,\sum_{t=1}^T\,\cL_1(\bxi, \blambda^t) \,+\, 
% \cO\left(\frac{1}{\sqrt{T}}\right).
4L\sqrt{\frac{\log(d)}{T}}.
\label{eq:gda-unc-xi-regret}
\end{eqnarray}
Combining \eqref{eq:gda-unc-lmo} and \eqref{eq:gda-unc-xi-regret}, we have with probability at least $1-\delta$ (over draw of $S$):
\begin{eqnarray}
\frac{1}{T}\sum_{t=1}^T\cL(\C^t, \bxi^t, \blambda^t)&\leq&
\min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\sum_{t=1}^T\,\cL(\C, \bxi, \blambda^t) \,+\, 4L\sqrt{\frac{\log(d)}{T}} \,+\, L\rho \,+\, L\rho'
\nonumber
\\
&=&
\min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C, \bxi, \bar{\blambda}) \,+\, 4L\sqrt{\frac{\log(d)}{T}} \,+\, L\rho \,+\, L\rho'
\nonumber
\\
&\leq&
\max_{\blambda \in \Lambda}\min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C, \bxi, {\blambda}) \,+\, 4L\sqrt{\frac{\log(d)}{T}} \,+\, L\rho \,+\, L\rho'
\nonumber\\
&=&
\min_{\C\in\cC}\left\{\max_{\blambda \in \Lambda}\,\min_{\bxi\in[0,1]^d}\,\cL(\C, \bxi, {\blambda})\right\} \,+\, 4L\sqrt{\frac{\log(d)}{T}} \,+\, L\rho \,+\, L\rho'
\nonumber\\
&=&
\min_{\C\in\cC}\psi(\C) \,+\, 4L\sqrt{\frac{\log(d)}{T}} \,+\, L\rho \,+\, L\rho'
\nonumber\\
&=&
\psi(\C^*) \,+\, 4L\sqrt{\frac{\log(d)}{T}} \,+\, L\rho \,+\, L\rho',
\label{eq:gda-unc-C-xi}
\end{eqnarray}
where in the second step $\bar{\blambda} = \frac{1}{T}\sum_{t=1}^T\blambda^t$ and we use the linearity of $\cL$ in $\blambda$; in the fourth step we use strong duality to interchange the max and min; and in the last step we apply Lemma \ref{lem:gda-unc-helper}.

Similarly, we apply the analysis for exponentiated gradient \textit{ascent}  on the sequence of losses $\cL(\C^t, \bxi^t, \cdot)$'s, where the optimization is over $\blambda$. Because $\|\nabla_{\blambda} \cL(\C^t, \bxi^t,\blambda^t)\|_2 = \|\C^t - \bxi^t\|_\infty \leq 1$, with $\eta' = \frac{1}{L}\sqrt{\frac{\log(d)}{T}}$, we have:
\begin{eqnarray}
\frac{1}{T}\sum_{t=1}^T\cL(\C^t, \bxi^t, \blambda^t) &\geq&
\max_{\blambda \in \Lambda}\,\sum_{t=1}^T\,\cL(\C^t, \bxi^t,\blambda) \,-\, 2L\sqrt{\frac{\log(d)}{T}}
\nonumber
\\
&\geq&
\max_{\blambda \in \Lambda}
\left\{
\sum_{t=1}^T\,\cL(\C[h^t], \bxi^t,\blambda) 
\,-\,  \|\blambda\|_1\|\C^t - \C[h^t]\|_\infty
\right\}
\,-\, 2L\sqrt{\frac{\log(d)}{T}}
\nonumber
\\
&\geq&
\max_{\blambda \in \Lambda}\,
\sum_{t=1}^T\,\cL(\C[h^t], \bxi^t,\blambda) 
\,-\,  L\rho'
\,-\, 2L\sqrt{\frac{\log(d)}{T}}
\nonumber
\\
&\geq&
\max_{\blambda \in \Lambda}\,\cL(\C[\bar{h}], \bar{\bxi},\blambda) 
\,-\,  L\rho'
\,-\, 2L\sqrt{\frac{\log(d)}{T}}
\nonumber\\
&\geq&
\min_{\bxi\in [0,1]^d}\,\max_{\blambda \in \Lambda}\,\cL(\C[\bar{h}], {\bxi},\blambda)
\,-\,  L\rho'
 \,-\, 2L\sqrt{\frac{\log(d)}{T}}
\nonumber
\\
&=&
\psi(\C[\bar{h}])
\,-\,  L\rho'
\,-\, 2L\sqrt{\frac{\log(d)}{T}},
\label{eq:gda-unc-lambda}
\end{eqnarray}
where
in the third step, we use the fact that for any $\lambda \in \Lambda$,  $\|\blambda\|_1 \leq L$, and the property of the LMO. 
In the fourth step, we use 
$\C[\bar{h}] = \frac{1}{T}\sum_{t=1}^T \C[h^t]$ and $\bar{\bxi} = \frac{1}{T}\sum_{t=1}^T \bxi^t$, and use the linearity of $\cL$ in $\C$, and convexity of $\cL$ in $\bxi$ and Jensen's inequality. In the final step, we apply Lemma \ref{lem:gda-unc-helper}. The last four steps hold with probability at least $1-\delta$.

Combining \eqref{eq:gda-unc-C-xi} and \eqref{eq:gda-unc-lambda}, we get with probability at least $1-\delta$ (over draw of $S$).
\begin{eqnarray*}
\psi(\C[\bar{h}]) \leq \psi(\C^*) \,+\, 6L\sqrt{\frac{\log(d)}{T}} \,+\, L\rho \,+\, 2L\rho'.
\end{eqnarray*}
Setting $T=\log(d)/\epsilon^2$ completes the proof.
%%%
% \begin{eqnarray}
% \max_{\blambda \in \Lambda}\,\cL(\bar{\C}, \bar{\bxi},\blambda) 
% &\leq&
% \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\cL(\C, \bxi, \bar{\blambda}) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, L\rho \,+\, L\rho',
% \label{eq:gda-unc-combined}
% \end{eqnarray}
% which shows that $(\bar{\C}, \bar{\bxi}, \bar{\blambda})$ is an approximate saddle-point solution for the min-max problem in \eqref{eq:minmax-reformulation}.


% Now to complete our proof, we lower bound the LHS in \eqref{eq:gda-unc-combined} by plugging $\blambda = \0$ and upper bound the RHS of \eqref{eq:gda-unc-combined} by plugging in $\C = \bxi = \C^*$, giving us:
% \begin{eqnarray}
% \psi(\bar{\bxi})
% &\leq&
% \psi(\C^*) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, L\rho \,+\, L\rho'.
% \label{eq:gda-unc-final-1}
% \end{eqnarray}
% Next, let $k \in \argmax_{j \in [d]} |\bar{C}_j - \bar{\xi}_j|$ be an index where the slack vector $\bxi$ differs most from the confusion matrix $\bar{\C}$,
% and let $\blambda' \in \R^d$ be such that 
% $\lambda'_j = \lambda^*_j, \forall j \ne k$ and $\lambda'_k = \lambda^*_k + L\sign(\bar{C}_j - \bar{\xi}_j)$. Note that because $\|\blambda^*\|_1 \leq L$, $\|\blambda'\|_1 \leq 2L$ and therefore $\blambda' \in \Lambda$. Lower bounding the the LHS in \eqref{eq:gda-unc-combined} by plugging $\blambda = \blambda'$ and upper bounding the RHS of \eqref{eq:gda-unc-combined} by plugging in $\C = \bxi = \C^*$, we get:
% \begin{eqnarray*}
% \psi(\bar{\bxi}) \,+\, \langle \blambda^*, \bar{\C} - \bar{\bxi} \rangle \,+\, L|\bar{C}_k - \bar{\xi}_k|
% &\leq&
% \psi(\C^*) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, L\rho \,+\, L\rho',
% \end{eqnarray*}
% which further gives us:
% \begin{eqnarray*}
% \min_{\C\in\cC,\, \bxi\in[0,1]^d}\,\left\{ \psi({\bxi}) \,+\, \langle \blambda^*, {\C} - {\bxi} \rangle
% \right\} \,+\, L|\bar{C}_k - \bar{\xi}_k|
% &\leq&
% \psi(\C^*) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, L\rho \,+\, L\rho'
% \end{eqnarray*}
% or
% \begin{eqnarray*}
% \psi(\C^*) \,+\, L|\bar{C}_k - \bar{\xi}_k|
% &\leq&
% \psi(\C^*) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, L\rho \,+\, L\rho'
% \end{eqnarray*}
% or
% \begin{eqnarray}
% \max_{j \in [d]}|\bar{C}_j - \bar{\xi}_j|
% &\leq&
% \cO\left(\frac{1}{L\sqrt{T}}\right) \,+\, \frac{\rho}{L} \,+\, 2\rho'.
% \label{eq:gda-unc-final-2}
% \end{eqnarray}
% Substituting from \eqref{eq:gda-unc-final-2} into \eqref{eq:gda-unc-final-1} and using the fact that $\psi$ is $L$-Lipschitz w.r.t.\ the $\ell_1$-norm, we finally have:
% \begin{eqnarray*}
% \psi(\bar{\C})
% &\leq&
% \psi(\C^*) \,+\, \cO\left(\frac{1}{\sqrt{T}}\right) \,+\, 2\rho \,+\, 4L\rho',
% \end{eqnarray*}
% which completes the proof.
\end{proof}

==> temp.tex <==
\subsection{Proof of Theorem \ref{thm:bisection-unc} (Bisection For Unconstrained Problems)}
\begin{thm*}[(Restated )Convergence of Bisection algorithm]
Fix $\epsilon \in (0,1)$. 
Let $\psi: [0,1]^d \> [0,1]$ be such that $\psi(\C) \,=\, \frac{\langle \A, \C \rangle}{\langle \B, \C \rangle}$, where $\A, \B \in \R^{n \times n}$, %. Moreover, assume $\inf_{\C \in \cC}\,\psi(\C) \,\leq\, 1$, 
and $\min_{\C \in \cC} {\langle \B, \C \rangle} \,=\, b$ for some $b > 0$. Let $\Omega$ in Algorithm \ref{alg:bisection} be a $(\rho , \rho', \delta)$-approximate LMO for sample size $N$.
Let $\bar{h}$ be a classifier returned by Algorithm \ref{alg:bisection} when run for $T$ iterations. % with a sample $S \sim D^m$. 
 Then with probability $\geq 1 - \delta$ over draw of $S \sim D^N$, after $T = \log(1/\epsilon)$ iterations:
\[
\psi(\C[\bar{h}]) \,\leq\, \min_{\C \in \cC}\,\psi(\C) \,+\,\cO\left(\epsilon + \kappa(\rho + \rho')\right),
\]
where $\kappa = \frac{1}{b}(\|\A\|_1 + \|\B\|_1)$.
\end{thm*}

 We will find it useful to state the following lemmas:
\begin{lem}[\textbf{Invariant in Algorithm \ref{alg:bisection}}]
\label{lem:lower-upper-bounds}
Under the assumptions made in Theorem \ref{thm:bisection-unc}, the following invariant is true at the end of each iteration $0 \leq t \leq T$ of Algorithm \ref{alg:bisection}:
\[
\alpha^t  - \kappa\bar{\epsilon} \,\leq\, \min_{\C \in \cC} \psi(\C) \,\leq\, \psi(\C[h^t])  \,<\, \beta^t + \kappa\bar{\rho},
\]
where $\kappa = \frac{1}{b}(\|\A\|_1 + \|\B\|_1)$ and
$
\bar{\rho} \,=\, \rho + \rho'.
$
\end{lem}

\begin{proof}
% We first have from Lemma \ref{lem:regret-bound-linear-psi-est-cond-prob}, the following guarantee for the linear minimization step at each iteration $t$ of Algorithm \ref{algo:BS}:
% \begin{eqnarray}
%  \langle\widehat{\L}^t,\, \C^D[\widehat{g}^t] \rangle  &\leq& \min_{\C \in \cC_D} \langle \widehat{\L}^t,\, \C \rangle  \,+\, \E_X\big[\big\|\widehat{\boldeta}(X) \,-\, \boldeta(X)\big\|_1\big] \nonumber\\
%  &=& \min_{\C \in \cC_D} \langle \widehat{\L}^t,\, \C \rangle  \,+\, \epsilon \hspace{0.5cm}\text{(say)}.
% \label{eqn:bs-lmo-1}
% \end{eqnarray}
% Further, let us denote $\epsilon' \,=\, \sup_{h \in \H_\boldeta}\|\C^D[h] \,-\,  \widehat{\C}^{S_2}[h]\big\|_\infty$. Notice that $\bar{\epsilon} = \epsilon + \epsilon'$.
%
%Further, applying the uniform convergence bound in Lemma \ref{lem:uconvg} to the confusion matrix estimate $\widehat{\bGamma}^t = \widehat{\C}^{S_2}[h^t]$ from partition $S_2$ of $S$ (of size $m/5$), we have for any fixed $\delta >0$, with probability at least $1-\delta$ (over draw of $S$ from $D^m$), at each iteration $0 \leq t \leq T$ of Algorithm \ref{algo:BS},
%\begin{eqnarray}
%\|\C^D[\widehat{g}^t] \,-\, \widehat{\bGamma}^t\big\|_\infty \,\,\leq\,\, \sqrt{2}C\sqrt{\displaystyle\frac{n^2\log(n)\log(m) + \log(n^2/\delta)}{m}}
%\,\,=\,\, \epsilon' \hspace{0.5cm}\text{(say)}
%\label{eqn:bs-lmo-2}
%\end{eqnarray}
%for some distribution-independent constant $C > 0$. Notice that $\bar{\epsilon} = \epsilon + \epsilon'$.
%
We shall prove this lemma by mathematical induction on the iteration number $t$. For $t=0$, the invariant holds trivially as $0 \leq \psi(\C[h^0]) \leq 1$. Assume the invariant holds at the end of iteration $t-1 \in \{0, \ldots, T-1\}$; we shall prove that the invariant holds at the end of iteration $t$. In particular, we consider two cases at iteration $t$. In the first case, $\psi(\C^t) \leq \gamma^t$, leading to the assignments $\alpha^t = \alpha^{t-1}$, $\beta^{t} = \gamma^t$, and $h^{t} = g^t$. We have from the property of the LMO (in Definition \ref{defn:lmo}) that:
% from the definition of $\epsilon'$
\begin{eqnarray*}
\langle \A - \gamma^t\B,\,\C[{g}^t]) \rangle
&\leq& \langle \A - \gamma^t\B, \,\C^t \rangle
  \,+\, \|\A - \gamma^t\B\|_1\rho'\\
&=& \langle \A,\,\C^t \rangle \,-\, \gamma^t\langle \B,\,\C^t \rangle 
  \,+\, \|\A - \gamma^t\B\|_1\rho'\\
&=& \langle \B,\,\C^t \rangle \big(\psi^\rl(\C^t) \,-\, \gamma^t\big)
  \,+\, \|\A - \gamma^t\B\|_1\rho\\
&\leq& 0 \,+\, \|\A - \gamma^t\B\|_1\rho'\\
&<& \|\A - \gamma^t\B\|_1(\rho + \rho')\\
&\leq& (\|\A\|_1 + \|\B\|_1)\bar{\rho},
\end{eqnarray*}
where the third step follows from our case assumption that $\psi^\rl(\C^t) \leq \gamma^t$ and $\langle \B,\,\C^t \rangle > 0$, the fifth step follows from $\rho > 0$, and the last step follows from triangle inequality and $0 \leq \gamma^t \leq 1$. The above inequality further gives us
\begin{eqnarray*}
\frac{\langle  \A,\, \C[{g}^t] \rangle}{\langle \B,\, \C[{g}^t] \rangle} 
&<& \gamma^t \,+\, \frac{\|\A\|_1 + \|\B\|_1}{\langle \B, \C[{g}^t]\rangle}\bar{\rho}\\
&\leq& \gamma^t \,+\, \frac{1}{b}(\|\A\|_1 + \|\B\|_1)\bar{\rho}\\
&=& \gamma^t \,+\, \kappa\bar{\rho}\\
&=& \beta^t \,+\, \kappa\bar{\rho},
\end{eqnarray*}
where the second step follows from $\underset{\C \in \cC}{\min}\langle \B, \,\C \rangle > b$ and the last step follows from the assignment $\beta^t = \gamma^t$. In other words,
\[
\psi^\rl\big(\C[h^{t}]\big) \,=\, \psi^\rl(\C[{g}^t]) \,=\, \frac{\langle \A,\, \C^D[{g}^t] \rangle}{\langle \B,\, \C^D[{g}^t] \rangle}  \,<\, \beta^t \,+\, \kappa\bar{\rho}.
\]
Moreover, by our assumption that the invariant holds at the end of iteration $t-1$, we have
\[
\alpha^{t} \,-\, \kappa\bar{\rho} \,=\, \alpha^{t-1} \,-\, \kappa\bar{\rho}  \,\leq\, \min_{\C \in \cC}\psi^\rl(\C) \,\leq\, \psi^\rl(\C[h^{t}]) \,<\, \beta^t \,+\, \kappa\bar{\rho}.
\]
Thus under the first case, the invariant holds at the end of iteration $t$.

In the second case, $\psi^\rl(\C^t) > \gamma^t$ at iteration $t$, which would lead to the assignments $\alpha^t = \gamma^{t}$, $\beta^{t} = \beta^{t-1}$, and $h^{t} = h^{t-1}$. Since the invariant is assumed to hold at the end of iteration $t-1$, we have
\begin{equation}
\label{eqn:case-2-partial}
\beta^t + \kappa\bar{\rho} \,=\, \beta^{t-1} + \kappa\bar{\rho}  \,>\, \psi^\rl(\C[h^{t-1}]) \,=\, \psi^\rl(\C[h^{t}]).
\end{equation}
Next, %recall that ${\L}^t \in [0,1]^{n\times n}$ is a scaled and translated version of $-(\A - \gamma^t\B)$; clearly, there exists $c_t \in \R$ and  $0 < a_t \leq 2\|\A - \gamma^t\B\|_\infty$ such that $\A - \gamma^t\B = c_t -  a_t \L_t$.
let $a_t = \|\A - \gamma^t\B\|_2$. 
Then for $\C^* \,\in\, \underset{\C \,\in\, \cC}{\argmin}\,\, \langle \A - \gamma^t\B, \,\C \rangle$, we have
\begin{eqnarray*}
\langle \A - \gamma^t\B, \,\C^* \rangle 
&=& a_t\langle {\L}^t, \,\C^* \rangle\\
&\geq& a_t\langle {\L}^t, \C[h^t] \rangle \,-\, a_t \rho\\
&\geq&a_t\langle {\L}^t, \C[h^t] \rangle \,-\, \|\A - \gamma^t\B\|_2 \rho\\
&=& \langle \A - \gamma^t\B, \,\C[h^t] \rangle  \,-\, \|\A - \gamma^t\B\|_2 \rho\\
%&=& \frac{1}{\|\A - \gamma^t\B\|_\infty}\langle \A - \gamma^t\B, \,\conf(\widetilde{h}^j, D) \rangle \,+\, \epsilon\\
%&=& \langle \A - \gamma^t\B, \,\conf(\widetilde{h}^j,D) \rangle \,+\, \|\A - \gamma^t\B\|_\infty \epsilon\\
&\geq& \langle \A - \gamma^t\B, \,\C^t \rangle \,-\, \|\A - \gamma^t\B\|_\infty\|\C^t - \C[h^t]\|_1 \,-\, \|\A - \gamma^t\B\|_2 \rho\\
&\geq& \langle \A - \gamma^t\B, \,\C^t \rangle \,-\, \|\A - \gamma^t\B\|_\infty\rho' \,-\, \|\A - \gamma^t\B\|_2 \rho\\
&=& \langle \A, \,\C^t \rangle - \gamma^t\langle\B, \, \C^t\rangle
  \,-\, \|\A - \gamma^t\B\|_\infty\rho' \,-\, \|\A - \gamma^t\B\|_2\rho\\
&=& \langle\B, \, \C^t\rangle(\psi(\C^t) - \gamma^t)
  \,-\, \|\A - \gamma^t\B\|_\infty\rho' \,-\, \|\A - \gamma^t\B\|_2\rho\\
&\geq& \langle\B, \, \C^t\rangle(0)
  \,-\, \|\A - \gamma^t\B\|_\infty\rho' \,-\, \|\A - \gamma^t\B\|_2\rho\\
&\geq& -\|\A - \gamma^t\B\|_1\bar{\rho}\\
&\geq& -(\|\A\|_1 + \|\B\|_1)\bar{\rho},
\end{eqnarray*}
where the second step follows from the property of the LMO, the sixth step follows from Holder's inequality and the property of the LMO, the ninth step follows from our case assumption that $\psi^\rl(\C^t) \geq \gamma^t$ and $\langle\B, \, \C^t\rangle > 0$, and the last step follows from triangle inequality and $0 \leq \gamma^t \leq  1$. In particular, we have for all $\C \in \cC$,
\[
\langle \A - \gamma^t\B, \,\C \rangle  \,\geq\, -(\|\A\|_1 + \|\B\|_1)\bar{\rho},
\]
or
\[
\frac{\langle \A, \,\C \rangle}{\langle \B, \,\C \rangle} \,\geq\, \gamma^t \,-\, \frac{\|\A\|_1 + \|\B\|_1}{\langle \B, \,\C \rangle}\bar{\rho}.
\]
Since $\underset{\C \in \cC}{\min}\langle \B, \,\C \rangle = b$, we have from the above, for all $\C \in \cC$,
\[
\psi^\rl(\C) \,\geq\, \gamma^t \,-\, \frac{1}{b}(\|\A\|_1 + \|\B\|_1)\bar{\rho} \,=\, \alpha^t - \kappa\bar{\rho}.
\]	
In other words, 
\[
\min_{\C \in \cC_D}\psi^\rl(\C) ~\geq~ \alpha^{t} - \kappa\bar{\rho}.
\]
By combining the above with \Eqn{eqn:case-2-partial}, we can see that the invariant holds in iteration $t$ under this case as well. This completes the proof of the lemma.
\end{proof}

\begin{lem}[\textbf{Multiplicative Progress in Each Iteration of Algorithm \ref{alg:bisection}}]
\label{lem:multiplicative-progress}
Let $\psi$ be as defined in \Thm{thm:BS-consistency}. Then the following is true in each iteration $1 \leq t \leq T$ of Algorithm \ref{alg:bisection}: 
\[
\beta^t - \alpha^t ~=~ \frac{1}{2}\big(\beta^{t-1} - \alpha^{t-1}\big)	.
\]
\end{lem}

\begin{proof}
We consider two cases in each iteration of Algorithm \ref{alg:bisection}. If in an iteration $t \in \{1, \ldots, T\}$, 
$\psi^\rl(\C^t) \leq \gamma^t$, leading to the assignment $\beta^t = \gamma^t$, then
\begin{eqnarray*}
\beta^t - \alpha^t &=& \gamma^t - \alpha^{t-1}\\
&=& \frac{\alpha^{t-1} + \beta^{t-1}}{2} - \alpha^{t-1}\\
&=& \frac{1}{2}(\beta^{t-1} - \alpha^{t-1}).
\end{eqnarray*}
On the other hand, if
$\psi^\rl(\C^t) > \gamma^t$, leading to the assignment $\alpha^t = \gamma^t$, then
\begin{eqnarray*}
\beta^t - \alpha^t &=& \beta^{t-1} - \gamma^t\\
&=& \beta^{t-1} - \frac{\alpha^{t-1} + \beta^{t-1}}{2}\\
&=& \frac{1}{2}\big(\beta^{t-1} - \alpha^{t-1}\big).
\end{eqnarray*}
Thus in both cases, the statement of the lemma is seen to hold.
\end{proof}

We are now ready to prove Theorem \ref{thm:bisection-unc}.

\begin{proof}[of Theorem \ref{thm:bisection-unc}]
For the classifier $\bar{h} = h^T$ output by Algorithm \ref{alg:bisection} after $T$ iterations, we have from \Lem{lem:lower-upper-bounds},
\begin{eqnarray*}
\psi^\rl\big(\C[h^T]\big) \,-\,
\min_{\C \in \cC_D} \psi^\rl(\C)
&< & (\beta^t \,+\, \kappa\bar{\rho}) \,-\, (\alpha^t \,-\, \kappa\bar{\rho})\\
&=& \beta^t - \alpha^t \,+\, 2\kappa\bar{\rho}\\
&\leq& 2^{-T}\big(\beta^0 - \alpha^0\big) \,+\, 2\kappa\bar{\rho}\\
&=& 2^{-T}\big(1 - 0\big) \,+\, 2\kappa\bar{\rho}\\
&=& 2^{-T} \,+\, 2\kappa\bar{\rho},
\end{eqnarray*}
where $\bar{\epsilon}$ is as defined in \Lem{lem:lower-upper-bounds}; the fifth step above follows from Lemma \ref{lem:multiplicative-progress}. Setting $T = \log(1/\epsilon)$ completes the proof.
\end{proof}
